mmFlexible: Flexible Directional Frequency Multiplexing for Multi-user mmWave Networks

Modern mmWave systems have limited scalability due to inflexibility in performing frequency multiplexing. All the frequency components in the signal are beamformed to one direction via pencil beams and cannot be streamed to other user directions. We present a new flexible mmWave system called mmFlexible that enables flexible directional frequency multiplexing, where different frequency components of the mmWave signal are beamformed in multiple arbitrary directions with the same pencil beam. Our system makes two key contributions: (1) We propose a novel mmWave front-end architecture called a delay-phased array that uses a variable delay and variable phase element to create the desired frequency-direction response. (2) We propose a novel algorithm called FSDA (Frequency-space to delay-antenna) to estimate delay and phase values for the real-time operation of the delay-phased array. Through evaluations with mmWave channel traces, we show that mmFlexible provides a 60-150% reduction in worst-case latency compared to baselines

==> Arxiv/1_intro_v1.tex <==
% !TEX root = main.tex
\section{Introduction}\label{sec:intro}

% New in intro_v3: Don't bring OFDMA, don't bring hybrid array. Just focus on TDMA, requirements for scalability, and split-antenna baseline.
% \todo{New pitch for intro_v4: Don't bring scalability but bring flexibility and resource efficiency (percent bandwidth usage). }
% New for Infocom v1: Pitch for flexible frequency multiplexing and how it helps with 1. diverse traffic, latency, and throughput due to flexible OFDMA

% A key trend for the next generation cellular networks is the growing number of devices and the diversity of applications ranging from latency sensitive URLLC to throughput intensive emBB video streaming applications. As the sub-6 spectrum is getting overcrowded, the new mmWave spectrum with high bandwidth has abundant opportunity to scale the wireless connectivity to the next billion devices. 

% Scaling wireless connectivity to a growing number of users requires judiciously using the time, frequency, and space resources to serve those users in the network. 
% Surprisingly, unlike the sub-6 counterpart, millimeter-wave (mmWave) networks cannot perform \textit{flexible directional frequency multiplexing} despite massive bandwidth at these frequencies, i.e., they cannot distribute small chunks of contiguous frequency bands to multiple users concurrently, where each user is in a disparate direction. The reason for this inflexibility is that the mmWave system creates a pencil beam that illuminates a small region in space. It means all the frequency components are radiated towards one fixed direction and cannot be distributed to other directions. It has two negative implications, as shown in Fig. \ref{fig:TDMA_OFDMA_3D}(a):
% 1. High latency: As the gNB has hundreds of pencil beams to cover the user space, some users have to wait long for their turn to get served, thus detrimental to latency-sensitive applications.
% 2. Low effective spectrum usage: When the aggregate demand in one direction is low, a small frequency band would be enough to serve users in that direction, but because the gNB can not radiate the rest of the frequency resources to another direction, those resources are wasted, leading to low effective spectrum usage. Moreover, other users in other directions could have used those wasted bands to improve the spectrum usage. 

Millimeter-wave (mmWave) networks have the potential to provide wireless connectivity to a growing number of users with their vast bandwidth resources. However, current mmWave systems have a significant limitation that they are unable to simultaneously serve multiple users by distributing small chunks of frequency resources to different users who are in different directions. This is because mmWave systems use pencil beams that illuminate a small region in space, meaning that all the frequency components are directed towards a fixed direction and cannot be distributed to other directions. This inflexibility leads to two main issues, as illustrated in Figure \ref{fig:TDMA_OFDMA_3D}(a). Firstly, it leads to high latency, as the base station (gNB) must scan a large number of pencil beams over time to serve all users, causing some users to experience long wait times, which is detrimental to latency-sensitive applications. Secondly, it leads to low effective spectrum usage. When demand in a particular direction is low, a small frequency band would be sufficient to meet the demand, but because the gNB cannot direct the remaining frequency resources to other directions, those resources are wasted, leading to low effective spectrum usage. Additionally, other users in other directions could have used these wasted bands to improve overall spectrum usage.



% A popular way to serve multiple users in sub-6 is time and frequency multiplexing, but surprisingly, it's extremely hard to do frequency multiplexing at mmWave frequencies. The root cause of this inflexibility lies in the different type of front-end architecture used for communication
% mmWave band and tera Hz band has huge spectrum with GHz of bandwidth but despite huge bandwidth, they don't scale well to a large number of users and diverse traffic scenarios. 
% mmWave uses directional beams to serve user locations which illuminate only a small fraction of area at a time. So the gNB scan beams over multiple TTI to serve data to more users. This way of time multiplexing or TDMA has two problems - it serves users sequentially and thus users have to wait for their turn to be served, 100s of directions in 3D space. 2. When the aggregate demand in one direction is low, only a few subcarriers are used to serve

% Unlike sub-6 omni-directional or sector-based antenna front-end, the mmWave front-end consists of a phased array with multiple antenna elements which focus the signal to a specific direction using a narrow pencil-beam. The phased array is fundamentally incapable of radiating different frequency components in the signal to different directions, i.e., all the frequency bands are transmitted in one direction even though the aggregate demand in that direction is not enough. It scans beams and adds latency. 


% A naive solution to reduce latency is to split the antenna array into multiple sub-arrays and let each sub-array radiate the signal in multiple directions. But, this split-antenna array tradeoffs throughput for low latency as the antenna gain reduces by half with every split. Nonetheless, split-antenna array can still can't perform flexible frequency multiplexing like sub-6. 

% The incapability to use vast frequency resources for scaling to large users demand novel architectures

In this paper, we ask the question: ``\textit{can a mmWave base station take an arbitrary set of $K$ contiguous frequency bands and transmit/receive to any arbitrary set of $K$ directions (i.e., create an arbitrary frequency-direction response)?}". The above is easily achievable in sub-6 using massive antennas with digital beamforming; traditional mmWave systems relies on analog phased arrays with single RF-chain for cost and power efficiency. Analog phased array cannot create such arbitrary frequency-direction response because they take a single input from the RF-chain and radiate all frequency components in the signal 
% \todo{not clear, because they take single RF chain output and .... call analog array or analog beamforming not both.} 
% they feed a constant phase per antenna which is the same for all frequency components. So all frequency components radiate 
in one fixed direction. One naive way to radiate signal in multiple directions is to split the phased array into multiple sub-arrays and program the phase shifters in each sub-array to radiate in different directions. But, this solution would reduce the directivity in that direction due to a limited number of antennas, reducing signal strength, range, reliability, and even data rate. 
Our \dpa differs from the traditional \ttd array, which uses a fixed set of delays at each antenna to create a fixed prism-like pattern, i.e., distributing a fixed sub-set of frequencies in each direction without any flexibility and control~\cite{li2022rainbow}. The problem with this approach is that some frequency subcarriers are wasted in directions without active users, and the active user receives a tiny fraction of bandwidth in one timeslot (TTI), which may not meet the user demand in a reasonable time frame. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/intro_frequency_multiplexing.pdf}
    \caption{\name extends directional frequency multiplexing to multiple concurrent directions providing low latency and higher effective spectrum usage for mmWave cellular networks. }
    % \name enables frequency multiplexing to multi-user mmWave networks with high flexibility and resource-efficiency.
    % \caption{\name improves scalability and resource-efficiency of mmWave networks while maintaining high throughput and enables OFDMA with frequency-selective multi-beamforming technique to serve multiple users simultaneously.}
    \label{fig:TDMA_OFDMA_3D}
\end{figure}

In contrast, we present our system called \name, which performs \textit{flexible directional frequency multiplexing} by transmitting/receiving a sub-set of contiguous frequency resources to each user irrespective of their directions, until all of the resources allocated are used up (no spectrum wastage). Said differently, rather than transmitting all frequency components to one fixed direction, \name creates multiple concurrent pencil beams in different directions; Each beam carries a separate sub-set of frequency components for users in that beam direction, while other beams serve other directions with different frequency bands without compromising the beamforming gain in each direction. The set of frequency-direction pairs can be chosen arbitrarily, allowing flexibility in performing directional frequency multiplexing. 
It allows packing the entire frequency band (up to 800 MHz for 5G NR and 2.3 GHz for IEEE 802.11ax bands) with data to serve multiple users concurrently; thus reducing spectrum wastage and providing low latency to access the network, as shown in Fig. \ref{fig:TDMA_OFDMA_3D}(b). 



% which utilizes the large bandwidth at mmWave frequencies to perform flexible frequency multiplexing. A key requirement for \name is to create multiple directional beams where different directions carry different frequency components for different users concurrently, thus creating a frequency-selective multi-beamforming patterns. 
% It allows multiple users to be served over multiple frequency bands in the same TTI, thus reducing the latency and improving the spectrum usage as shown in Fig. \ref{fig:TDMA_OFDMA_3D}(b). 

% \todo{you need to rework the next two paragraph, you are done bunch of back and forth... }
% The natural question is how does \name creates such "flexible" frequency-space patterns? A key insight for \name is to use a analog delay element at each antenna to achieve frequency selectivity.  The delay element creates different phase for different frequency and so radiates different frequency in different directions. \name's architecture consists of designing novel \dpa, an antenna array design that can construct arbitrary and controllable frequency-selective multi-beams, which can enable slicing of frequency resources and radiating each resource as pencil-beam to any desired directions simultaneously. 

% Creating a \ttd element has been popularly used for mmWave antenna arrays for fast beamforming and solving beam squinting issues. In contrast, \name is the first work to propose using delay element for a different application of flexible frequency multiplexing.

% One of the biggest challenge for \name is to create arbitrary and controllable frequency-selective beams using \dpa. It means the array should be able to serve an arbitrary set of user directions with an arbitrary size of frequency bands allocated to each user. 

A natural question is how does \name create analog beamforming to serve arbitrary frequency-direction pairs? We design a novel mmWave analog array architecture called \dpa, which implements a variable delay and phase element to create any desired frequency-direction response. 
In contrast to the fixed delay architecture, our \dpa tunes variable delay and variable phase to achieve flexibility in choosing which direction to serve and over what bands arbitrarily. Our insight is to use delays and phases in a complementary manner:  the variable delay provides \textit{frequency-selectivity}, and the variable phase provides direction steerability. \name deploys delay and phase together to create pencil beams towards multiple arbitrarily chosen frequency-direction pairs, thus creating any desired frequency-direction response. 





% A natural question is how does \name create such ``flexible" and arbitrary frequency-direction response? We design a novel mmWave front-end architecture called \dpa that uses a variable delay and a variable phase element at each antenna to achieve frequency selectivity. While a few works propose using the delay element in a true-time delay array~\cite{yan2019wideband, boljanovic2020design,wadaskar20213d,boljanovic2020true,boljanovic2021fast}, we are the first to explore it in our \dpa architecture to create arbitrary and controllable frequency-selective multi-beams.
% We cannot use the traditional \ttd array for this problem because it creates a prism-like response that radiates a fixed sub-set of frequencies in each direction without any flexibility and control~\cite{li2022rainbow}. As a result, frequency resources are wasted in directions without active users. Even when there is an active user, the user receives a tiny fraction of the bandwidth in one timeslot (TTI), which may not meet the user demand in a reasonable time frame, thus compromising user throughput. In contrast, the key insight for \name is solving this challenge using variable delay and phase element in \dpa. The variable delay and phase element in \dpa tunes the beamforming response in a  complementary manner: the variable delay provides frequency-selectivity, and the variable phase provides direction steerability. In this paper, we show how our \dpa uses these two elements to combine the two worlds of frequency and direction to create flexible frequency-selective multi-beams, i.e., we can arbitrarily and flexibly transmit/receive any amount of bandwidth in any direction to use up the entire allocated spectrum with energy efficient analog \dpa architecture.

We architect our \dpa and provide valuable insights on the hardware requirements for creating these antenna arrays. We perform the range and resolution analysis on \dpa to arbitrarily and flexibly transmit/receive any amount of bandwidth in any direction and use the entire spectrum. Implementing large delays on circuits as large transmission lines is size prohibitive and integrating them onto an IC is even more challenging in mmWave due to bandwidth and matching constraints~\cite{ghaderi2019integrated}. Therefore, we design to ensure that the requirement on the range of delay values is significantly lower than that suggested in the literature for other \ttd applications~\cite{li2022rainbow}. \ttd array applications require monotonic increasing delays at each antenna; for even a 16 element array, the delay requirement is 20 ns, 13x more than state of art mmWave delay design~\cite{ghaderi2019integrated}. In contrast, \dpa consists of increasing and decreasing delay values for consecutive antennas with a net effect of lower delay range requirements than traditional \ttd arrays. Moreover, the delay range is independent of the number of antenna elements for large arrays, making our design practical and easy to manufacture.

% The delay provides a \todo{I don't follow slope what slope as in "slope of phase?"}slope in frequency-space domain and the phase provides a constant shift. We showed that variable delay and phase element together provide flexibility to tune any arbitrary frequency-space image. \name comes up with a design of \dpa with appropriate variable delays and phases for each antenna. \todo{four principles of writing what is the problem, why is it hard, what is simple solution and what is your solution.... this and previous paragraph are not exciting, it should land... }

A natural next challenge during the operation of \name's array is to create the desired frequency selective multi-beam response. To achieve this response, it has to estimate values for variable delays and phases at each antenna. Furthermore, the optimization has to solve for the discrete variable delay and phase elements, which makes the problem non-convex and NP-hard. An exhaustive search over all possible delay and phase combinations at each antenna would be computationally challenging during real-time operation. Moreover, storing the delay and phase value for every possible frequency-space (directions) is impossible, as the combinations of frequency-space are innumerable ($10^{28}$). We develop a single-shot solution for the delays and phases by developing a transform from delay-antenna to frequency-space domain. We represent the desired frequency selective multi-beam response as a 2D image and develop a 2D transform that takes the desired frequency-space image and transforms it into 2D delay-antenna space. We then extract the corresponding delays and phases per-antenna from this image. Our algorithm only requires the angles for each user and corresponding frequency resources allocated to users in the current time slot. The typical 5G mmWave standard protocol estimates each user's direction by default, thus making our algorithm easy to deploy. 



% \todo{talk about your simulation and emulation results to evaluation efficacy of your performance...}

% \textbf{Contributions:} 
\noindent
\textit{{In summary, \name makes the following contributions}}:
\begin{itemize}
    \item \name is the first system that lays the requirements for flexible frequency multiplexing in the mmWave regime. We design a novel mmWave front-end architecture called delay-phased array that meets those requirements achieving higher spectrum usage, low latency, and scalability to support a large number of users.
    \item We develop a novel 2D transform and algorithm called FSDA (Frequency-space to delay-antenna) to estimate the delays and phases in real-time. 
    % \todo{talk about transform first and then algorithm}   % \item We present a simplified scheduler for mmWave MAC that builds on top of popular sub-6 proportional-fair scheduler with the ability to support more than one directional beams at the same time.
    \item We evaluate \name on real mmWave traces and show overall multi-user sum-throughput improvement by 3.9$\times$ compared to a \ttd array baseline~\cite{li2022rainbow}, 1.5$\times$ compared to split-antenna baseline, and 1.3$\times$ compared to phased array with time-division multiple access (TDMA) scheme. The worst case latency is reduced by 72\%.
\end{itemize}
% }
% In this paper, we argue that delay-phased arrays with the ability of creating frequency-selective beams have a wider implication in mmWave technology beyond 5G. For instance, \dpa can be used for single-shot beam scan to find initial user direction for all users 





% TTD arrays are popular in literature with many applications such as single-shot beam training with rainbow beams and beam squinting resolution for large bandwidths\cite{}. However, none of the past works with TTD discuss or solve the multi-user scalability problem. 


% We construct a new phased array architecture with both delay and phase elements (we call it \dpa) and show that it can efficiently allocate independent beams and frequency resources to multiple users simultaneously, thus enabling OFDMA for mmWave.





% One possible solution to this is the network slicing concept prevalent in LTE and sub-6 5G networks, which enables these diverse applications over different time-frequency resources sharing the same set of hardware. 
% Clearly, a critical requirement for network slicing is providing independent time-frequency resources for different applications. 

% Traditional mmWave protocols are designed for these applications in isolation. They don't work out together. 
% However, the directional nature of mmWave links do not permit the network slicing concepts to work in the 5G FR mmWave bands. 
% The key reason is that for network slicing concept to work at mmWave links, they need to be upgraded with flexibility across the space dimension.
% The reason being that, mmWave links are directional in nature and hence the time-frequency slots 
% The slicing is supposed to be independent of each other. But, current technology cannot schedule network resources to different network slices independently. For instance, low-latency packets for mission critical applications could bring down the data rates for video streaming packets significantly. On the other hand, high throughput video streaming packets would increase the latency for mission critical applications.

% \todo{Explain via Table~\ref{tab:baseline_technologies}}.
% Traditional mmWave technology use TDMA or hybrid arrays to schedule resources over time and beam-space respectively. However, they are both inefficient and unscalable to meet users demands. TDMA suffers from worse spectrum utilization and high latency for mmWave as the entire 400MHz band must be allocated to a single UE even if the user's demand is significantly low as in for URLLC applications. This is because a single phased arrays can serve in only one direction at a time and cannot serve users in other directions simultaneously (Fig. \ref{fig:TDMA_OFDMA_3D}(a)). 

% Even hybrid mmWave with multiple phased arrays is not a scalable architecture since it would require prohibitively large number of phased arrays and RF-chains to cover the space. For instance, with a beamwidth of $6^\circ$, it requires $360^\circ/6^\circ = 60$ phased arrays to cover the 360-space. Therefore, hybrid arrays are not scalable to multi-user mmWave systems. 
% \todo{Should we bring Fully-digital here as well?}.




% Split-antenna reaps off all the benefits of a phased array and makes the link unreliable and low-throughput. 
% For the first time, we provide a solution to OFDMA for scalable multi-user communication.
% Providing entire 400 MHz band to a user in one TTI is unreasonable as it has a long transmission time which increases the latency. 

% 5G mmWave requires high directional beams to overcome propagation loses and maintain a high throughput link. When multiple flows are scheduled in different frequency bands, it is required to maintain multiple directional beams for each flow. However, COTS mmWave devices relies on a phased array to create a single directional beam which cannot support multiple users in different geographical locations. A naive solution is to split antennas to create multiple simultaneous beams. However, this solution compromises the antenna gain as a smaller subset of antennas are used to create directional beams which in turn reduces the overall throughput. Therefore, split-antenna is not scalable to a large number of users. 
% In this paper, we ask if we can  support a large number of user devices through frequency slicing without compromising data rates for any user.

% Requirements\\


% \noindent
% TDMA - supports high data rates and manages beams well, but it introduces high latency which is critical for URLLC applications. \\
% FDMA - Can support low-latency applications but cannot create different beams for different frequency. So it compromises throughput by adapting wide beams.\\
% Fully-digital - Can create freq-dependent beams but not adopted by industry. Expensive and power hungry. \\







% \todo{Describe challenges, solutions, and contributions}.

% \subsection{Random text from \cite{miao2016joint}}
% In addition to higher throughput, the future 5G system also targets to lower latency and better spectrum efficiency. As such, it is desired that the mmWave system can schedule as many users as possible in the same transmission time interval (TTI). In addition to the shared frequency resources, the mmWave system is also limited by the restrictions of physical analog beamformer.

% Typically, a radio resource scheduler at the MAC layer determines the radio resource allocation to each scheduled UE in the current TTI. In the LTE system, the radio resource is defined in a time-frequency resource grid. In addition to the frequency resource allocation, the mmWave AP also needs to appropriately select the transmitted beams for the scheduled UE. Hence, the radio resources managed in the mmWave system can be characterized as a resource grid of three dimensions including time, frequency and beam domains.


% \todo{Practical problems in mmWave, mention that }

% Features of \name:
% \begin{enumerate}
%     \item Enables OFDMA for mmWave by creating independent frequency-space beams. Traditionally all frequencies are sent along a single beam.
%     \item Scalable to 100s of diverse users (VR + URLLC). Traditional TDMA is not scalable
%     \item Provides high throughput for VR and low latency to URLLC at the same time. Traditional schemes trade-off one for the other.
%     \item Power efficient using single phased array (compared to fully-digital system)
%     \item 5G NR compatible. Low overhead.
% \end{enumerate}


% Challenges:
% \begin{enumerate}
%     \item How to estimate delays and phases per-antenna
%     \item Understanding delay quantization and hardware challenges
%     \item Logic for scheduler - scalable to 100s of users
%     \item Explore single-shot beam training with TTD (Danejila's paper)
%     \item Challenge with blockage and mobility - it becomes easy to track beams with frequency-beam independence
% \end{enumerate}

==> Arxiv/2_motivation_v1.tex <==
% !TEX root = main.tex
\section{Background and Motivation}\label{sec:motivation}
% In this section, we would present the application requirements and show how user-scalabililty cannot be supported with traditional mmWave multiplexing, i.e. they lack mechanism to share the Gbps links among many-many users and applications. Next, we provide a primer on mmWave communication system and fundamental reason for inability in supporting multiplexing, like sub-6 GHz counterparts. We conclude by articulating that mmWave networks needs to support both time-frequency resource block creation, vis-a-vis by creation of frequency-selective multi-beams to bridge this gap.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/compare_baselines_motivation.pdf}
%     \caption{Throughput-latency trade-off for different mmWave technologies. \name breaks the trade-off providing high throughput and low latency with flexibility to work in diverse traffic scenarios.}
%     \label{fig:compare_baselines_motivation}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/baseline_architecture_and_heatmap.pdf}
    \caption{Comparison of different mmWave front-end architectures and corresponding frequency-space patterns they create. It shows the traditional phased array and split-antenna array create frequency-flat response, while \ttd array create frequency-selective rainbow-like pattern radiating in all directions. In contrast, our \dpa architecture provides flexibility to create arbitrary and controllable frequency-selective beams. Note all frequency-space heatmaps are simulated with 8 antenna array and plotted with the same x-axis (angle from $-90^\circ$ to $90^\circ$), y-axis (frequency from -200 MHz to 200 MHz) and colorbar (Antenna gain from 0 to 5 dB). }
    \label{fig:baseline_architecture_and_heatmap}
\end{figure*}
% New in v3: improve 3.2 first by removing all the maths and explain intuitively and then work in simplifying 3.1
% v4: Completely new way to put this section based on Dinesh's feedback. 2.1 Applications, resource inefficiency. 2.2 Sub-6 OFDMA is great but not possible with mmWave - hybrid, splitantenna baseline etc. 2.3 Our insight/motivation without giving delay architecture. Tell why you need it and not how you use it.
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conventional_frequency_flat_vs_ours.pdf}
%     \caption{Conventional mmWave may split the beam, but they reduce the SNR and still create frequency-flat response. In contrast, \name creates high SNR frequency-selective multibeams..}
%     \label{fig:conventional_frequency_flat_vs_ours}
% \end{figure}

% \subsection{Supporting multi-user applications with mmWave}
Let us look at how the current mmWave systems have tried to address the increasing demand for data-rates and new users and see where they lack and what are the requirements to overcome these limitations.
With exponential growth in use of wireless connectivity, a diverse set of applications have emerged. A variety of applications from AR/VR to V2X have a high disparity in their data-rate and latency demands. 
% On the one hand, there are latency-sensitive applications such as online gaming and vehicular communication, and on the other hand, there are throughput-intensive applications such as VR. 
For VR applications alone, the data-rate and latency demands vary based on video quality, rendering requirements and resolution ranging from 20 Mbps at 40fps for a simple 4k VR video streaming to 400fps at 1 Gbps for 8k on-headset tethered VR.
% It is envisioned that the high-frequency mmWave bands could support these high-throughput and frame-rate demanding applications with a large amount of spectrum available at these frequencies. Furthermore, today's mmWave deployment is mostly limited to being able to serve one user at a time slot, and then multiplex over time-slots to serve multiple users. 
% In each slot direction of the one user who is going to be served is illuminated by the mmWave beams. 

% There are two problems with this approach. First, the users must wait for their turn to be served, which causes large delays for high-throughput and high-frame rate applications like tethered VR.
% For instance, let us consider 
Consider an example where a base station is serving 100 different VR users, in a 10-90 split, where the 10 users are tethering 8k VR streams on headsets and need a 1Gbps link with $<8$msec latency requirements, while the rest 90 users are streaming 4k VR videos requiring 50Mbps links with $<25$msec latency.
Since, existing mmWave can only perform time-multiplexing, they have to serve each of the user in a different time slot, with protocol specified TTI (transmission-time interval) of 0.125msec \cite{pocovi2018achieving,zhang2019machine}. 
Hence, it would take 12.5ms to serve all the 100 users, which would violate the $>8$msec for the 10 users having 8k video requirements. 
% to serve the Gbps users the next frame leading to lags and frame drops.
% \todo{reads odd, use "significant" instead of very}
Secondly it leads to significant   spectrum wastage, for example the 90 users from the above scenario are served a 1Gbps link while their requirement is at best for a 50Mbps link, leading to spectral efficiencies as low as $5\%$.
Thus scaling up the current mmWave systems to multiple users for these targeted applications is not possible, as they cannot meet the latency requirements for the high throughput demanding VR applications and are highly inefficient in spectral resource utilization.

% For instance, a base station with a narrow $6^\circ$ beam would scan $360^\circ/6^\circ = 60$ directions in azimuth angle and roughly 4x more to cover the elevation angles. This large angular diversity may cause up to 100 ms delay, which is intolerable for applications such as online gaming, which requires 10-20 ms end-end latency. Secondly, due to disparity in user demands, some applications require as low as 20 Mbps. Still, the base station allocates the entire bandwidth (a multi Gbps connection) resource to this user leading to the wastage of precious spectrum resources.
% We take insights from sub-6 communication, which efficiently serves multiple users with flexible time-frequency multiplexing. Therefore, it is logical to extend these capabilities for mmWave links too to enable efficient multi-user communication.




%  \begin{figure*} [!t]
%     \subfigure{{\includegraphics[width=0.24\textwidth]{figures/tdma_heatmap.pdf}\label{fig:tdma_heatmap}}}
%     \subfigure{{\includegraphics[width=0.24\textwidth]{figures/split_heatmap.pdf}\label{fig:split_heatmap}}}
%     \subfigure{{\includegraphics[width=0.24\textwidth]{figures/rainbow_heatmap.pdf}\label{fig:rainbow_heatmap}}}
%     \subfigure{{\includegraphics[width=0.24\textwidth]{figures/fsda_heatmap.pdf}\label{fig:fsda_heatmap}}}
%     \caption{Heatmap images of Antenna Gain across frequency and space for (a) Phased array, (b) Split-antenna array, (c)  True-time delay array~\cite{li2022rainbow}, (d) \name's \dpa. It shows how four distinct users at angle $-30^{\degree}$, $0^{\degree}$, $30^{\degree}$, and $60^{\degree}$ are supported by different approaches in one TTI.}
%     \label{fig:heatmap_all}
%     % \vspace{2pt}
% \end{figure*}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/phased_array.pdf}
%     \caption{Shows traditional phased array architecture creates frequency-flat beams.}
%     \label{fig:phased_array}
% \end{figure}

\subsection{Current mmWave architectures are incapable for flexible frequency multiplexing}
Current millimeter-wave system can't perform flexible frequency multiplexing because they use an antenna array to beamform signal to a specific direction and can only serve that direction. Though a fully-digital beamforming architecture can create frequency-selective beams, they are not feasible for mmWave bands because of high power and complexity in laying hundreds of RF chains for each antenna element.
% The sub-6 systems can easily do frequency multiplexing because it uses an omnidirectional antenna to radiate in all directions and so the intended users can receive data in their assigned frequency band and discard data in other bands. When the gNB has multiple antennas in MIMO-OFDMA system, it is possible to digitally beamform different frequency bands to different users. But, mmWave MIMO system is impractical because of high power and complexity in laying hundreds of RF chains for each antenna element. 

In contrast, mmWave front-end consists of analog antenna array for beamforming. Three common analog array architectures are: phased array, split-antenna array and true-time delay array. Here we show how these three architectures fail to perform flexible frequency multiplexing and suffer from either low throughput or high latency when serving multiple users in the network as shown in Figure~\ref{fig:compare_baselines_motivation}. The phased array provide high throughput when there are only few high-traffic users, but fails in a mixed or low traffic scenarios. It wastes a lot of spectrum and suffers from low throughput and high latency. Split-antenna array compromises on throughput to provide low latency. Finally, \ttd array is on the other extreme where it can provide low latency for sensitive IoT applications, but suffers from extremely low data rates. In contrast, our \dpa provides flexibility to perform frequency multiplexing with highly directional pencil beams for all users leading to both high sum throughput and low latency.

\subsection{Primer on phased arrays and true-time delay arrays}

\textbf{Phased array:}
The phased array takes a single input from the digital chain, split into $N$ copies, phase-shifted and radiated from $N$ antennas (Fig. \ref{fig:baseline_architecture_and_heatmap}(a)). The input signal consisting of all frequency bands is radiated in space with a beam pattern given by:
% One of the reasons why current mmWave technology cannot achieve better quality of service is due to its inability to serve multiple users with flexible time-frequency multiplexing.
% Efficient frequency multiplexing is a viable way to serve multiple users in a resource efficient manner as only required set of frequency resources can be allocated to users along different directions without compromising the link quality in any given direction.
% However current mmWave technology cannot perform frequency multiplexing due to an inflexible analog front-end architecture. The mmWave front-end uses a phased array architecture connected to the baseband with a single wire interface as shown in Figure~\ref{fig:phased_array}. This phased array takes the input signal from baseband and radiates it into space. 
% While radiating the signal, each individual antenna has a phase-shifter that adds an additional phase shift to the signal.
% These additional phase shifts at each antenna combine the signal such that one fixed angle gets the highest antenna gain while severely suffering at other angles. This directional gain is enabled to provide reliable throughput link to the user by overcoming the high attenuation rates of mmWave signals.
% To put it simply, the gain pattern of a phased array with $N$ antennas is given by:
\begin{equation}
        G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)V(n,\theta)
\end{equation}
where the weights $w_{\text{phase}}(n) = e^{j\Phi_n}$ contains programmable phases $\Phi_n$ and   $V(n,\theta) = e^{-jn\pi\sin(\theta)}$, is a standard steering matrix transformation from antenna to space-domain\footnote{Note that $V(n,\theta) = e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$ depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$. We assume $d=\frac{\lambda}{2}$ and approximate the array response as $V(n,\theta) = e^{-jn\pi\sin(\theta)}$.}. Now, if we program the phases to create a directional beam at an angle say $\theta_0$, then all the same phase offset is applied to all the frequency components in the signal. Thus all of these frequencies can only radiate along that one angle and cannot be spread to other directions. Therefore, a phased array can serve only one directional user at a time and cannot perform frequency multiplexing with many users. Even split-antenna phased array (Fig. \ref{fig:baseline_architecture_and_heatmap}(b)) 


\noindent
\textbf{True-time delay array:} The \ttd array uses a delay element to replace the phase shifter as shown in Fig. \ref{fig:baseline_architecture_and_heatmap}(c). The delay element creates different delays to the input signal at each antenna before they get radiated in space. When multiple copies of these waveforms from each antenna are added at the receiver, they create a unique gain pattern as a function of frequency content of the signal. To understand it concretely, we define the  antenna weights with delay element as:
\begin{equation}
    w_{\text{phase}}(t,n) = \delta(t-\tau_n)
\end{equation}
where $\tau_n$ is the variable delay at antenna $n$ and $t$ is the time axis. 

Here we can intuitively understand that a time varying signal has a certain frequency response. Upon taking FFT of $\delta(t-\tau_n)$, we get $e^{j2\pi f\tau_n}$. We observe that the phase of this exponential term is frequency-dependent, or in other words, the delay element creates frequency-varying phase at each antenna element. Now how does this enables frequency-selectivity? Unlike traditional phased array which adds a constant phase across all frequencies, we see that here different frequency components experience a different phase shift at each antenna which will make them radiate in different directions. 

A natural question is whether this delay element can create a desired frequency-selective beams. Past work on \ttd array~\cite{yan2019wideband, boljanovic2020design,wadaskar20213d,boljanovic2020true,boljanovic2021fast} have shown that this architecture creates a prism-type response by radiating all the frequencies in all the directions in a linear fashion as shown in Figure~\ref{fig:baseline_architecture_and_heatmap}(c). This response has two major limitations: 1) most frequency bands would be wasted in space if there are no user in that direction and 2) each user gets a small frequency band and cannot scale it up arbitrarily. Due to these limitations, delay-only array is not suitable for flexible frequency multiplexing.




% This phased array consists of a pragrammable phase shifter at each antenna that modulates the signal with a tunable phase value. This phase modulation enables for directed 

% There is a single data input to the phased array which is radiated in space.So, all the frequency bands in the input data is transmitted to the same direction and cannot be separated into different directions. 



% To put it simply, for a phased array with $N$ antennas we can achieve a gain-pattern, $G(\theta)$  by tuning as follows:

% \begin{equation}
%         G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)V(n,\theta)
% \end{equation}
% where the weights at each antenna $w_{\text{phase}}(n)$ consists of  

% $V(n,\theta) = e^{-jn\pi\sin(\theta)}$, is a standard steering matrix transformation from antenna to space-domain\footnote{Note that $V(n,\theta) = e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$ depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$. We assume $d=\frac{\lambda}{2}$ and approximate the array response as $V(n,\theta) = e^{-jn\pi\sin(\theta)}$.}. 

% Further we can easily show that (more details in Appendix~\ref{sec:appendix}.1) $w_{\text{phase}}(n) = e^{jn\pi\sin(\theta_0)}$ are the individual antenna phase that are applied through a programmable phase-shifter at each antenna $n$ as shown in Figure 3 to beamform towards the desired user direction $\theta_0$. 

% Even if we use multiple phased arrays with multiple inputs from the baseband in a MIMO fashion, each MIMO array might send their data in different directions, but they still can't do frequency multiplexing. Each phased arrays in MIMO would still send the entire input data to one direction. So MIMO arrays are in this way complementary to our problem, they may reduce the number of direction to serve from a single array, but still very resource inefficient because they can't do frequency multiplexing. Fundamentally, we need a way to perform frequency multiplexing with a single antenna array.


% A naive way to serve multiple directions with a single phased array is to divide the array into multiple sub-arrays and program each sub-arrays to radiate in one direction each~\cite{hassanieh2018fast, abari2016millimeter,marjan2018split,aykin2019multi}. In this way the input data can be spread in multiple directions and each user can extract their corresponding frequency bands as shown in Figure~\ref{fig:phased_array}(c).
% % as shown in Figure~\ref{fig:conventional_frequency_flat_vs_ours}(a). 
% The issue with this split-antenna approach is that rather than sending one frequency band in one direction and another frequency band in other direction, it sends all the frequency bands to all the directions. As a result, the transmit power is spread at multiple locations in space and so each user gets low power. The mmWave systems loses all the gains due to directional links and severely reduces the throughput and link reliability.


% \subsection{Motivation for \name}


% % \review{R1: The presented motivation for multi-user data transmission is not convincing. Reviewer said no advantage in spectral efficiency.} \todo{Don't say we improve spectral efficiency, but mention that we allow flexible resource allocation and reduce latency.}
% We have seen above how most of the existing mmWave algorithms that phased array compromise on \textcolor{blue}{resource} efficiency and latency due to their inability to perform \textcolor{blue}{flexible frequency multiplexing}. The other split-antenna systems compromise on the net throughput by splitting the antenna arrays.  On the other hand, the \ttd array compromises on throughput to get low latency. Thus it is the need of the hour to develop a system that can perform flexible frequency multiplexing to achieve both high throughput and low latency. It would enable to allocate and transmit only the frequency resources that a user demands in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Figure~\ref{fig:TDMA_OFDMA_3D}(b)). 
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.

% Therefore, our goal is to selectively radiate in frequency-space axis, and not illuminate all direction for all frequencies as it would reduce range and throughput....\todo{talk about those two scenarios} but we want to localize the beam in both frequency and space dimensions.
% This localization across both frequency and space, only the frequency resources that a user demands are allocated to that user in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Figure~\ref{fig:TDMA_OFDMA_3D}(b)). 
% In this way, it can support many users with frequency-multiplexing without compromising on directional gains and maintaining high throughput and reliable mmWave links.
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.

==> Arxiv/2_motivation_v2.tex <==
% !TEX root = main.tex
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/baseline_architecture_and_heatmap.pdf}
    \caption{Comparison of different mmWave front-end architectures and corresponding frequency-space patterns they create. It shows the traditional phased array and split-antenna array create a frequency-flat response, while \ttd array creates a frequency-selective rainbow-like pattern radiating in all directions. In contrast, our \dpa architecture provides flexibility to create arbitrary frequency-direction response. 
    % Note all frequency-space heatmaps are simulated with 8 antenna arrays and plotted with the same x-axis (angle from $-90^\circ$ to $90^\circ$), y-axis (frequency from -200 MHz to 200 MHz), and colorbar (Antenna gain from 0 to 5 dB). 
    }
    \label{fig:baseline_architecture_and_heatmap}
\end{figure*}

\section{Background and Motivation}\label{sec:motivation}
% More in Infocom v2: Reverse primer and example.
% # New in Infocom v2: Provide short comparison with 3 baselines in table form. 
% New in v3: improve 3.2 first by removing all the maths and explain intuitively and then work in simplifying 3.1
% v4: Completely new way to put this section based on Dinesh's feedback. 2.1 Applications, resource inefficiency. 2.2 Sub-6 OFDMA is great but not possible with mmWave - hybrid, splitantenna baseline etc. 2.3 Our insight/motivation without giving delay architecture. Tell why you need it and not how you use it.

In this section, we would provide a primer on different analog antenna array architectures, which have a single baseband radio frequency (RF) chain and mechanism to best achieve flexibility in resource allocation to multiple users. Next, we would show a realistic example that none of the architecture can meet the requirements for flexible directional frequency multiplexing, and how our flexible \dpa architecture can meet these requirements. 


\subsection{Primer on phased arrays and true-time delay arrays}

\textbf{Phased array:}
The phased array takes a single input from the digital chain, split into $N$ copies, phase-shifted and radiated from $N$ antennas (Fig. \ref{fig:baseline_architecture_and_heatmap}(a)). The input signal consisting of all frequency bands is radiated in space with a beam pattern given by:
% One of the reasons why current mmWave technology cannot achieve better quality of service is due to its inability to serve multiple users with flexible time-frequency multiplexing.
% Efficient frequency multiplexing is a viable way to serve multiple users in a resource efficient manner as only required set of frequency resources can be allocated to users along different directions without compromising the link quality in any given direction.
% However current mmWave technology cannot perform frequency multiplexing due to an inflexible analog front-end architecture. The mmWave front-end uses a phased array architecture connected to the baseband with a single wire interface as shown in Fig.~\ref{fig:phased_array}. This phased array takes the input signal from baseband and radiates it into space. 
% While radiating the signal, each individual antenna has a phase-shifter that adds an additional phase shift to the signal.
% These additional phase shifts at each antenna combine the signal such that one fixed angle gets the highest antenna gain while severely suffering at other angles. This directional gain is enabled to provide reliable throughput link to the user by overcoming the high attenuation rates of mmWave signals.
% To put it simply, the gain pattern of a phased array with $N$ antennas is given by:
\begin{equation}\label{eq:phasedarraygain}
        G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)V(n,\theta)
\end{equation}
where the weights $w_{\text{phase}}(n) = e^{j\Phi_n}$ contains programmable phases $\Phi_n$ for antenna index $n (n\in [0,N-1])$ and   $V(n,\theta) = e^{-jn\pi\sin(\theta)}$, is a standard steering matrix transformation from antenna to space-domain\footnote{Note that $V(n,\theta) = e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$ depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$. We assume $d=\frac{\lambda}{2}$ and approximate the array response as $V(n,\theta) = e^{-jn\pi\sin(\theta)}$.}. Now, if we program the phases to create a directional beam at an angle say $\theta_0$, then all the same phase offset is applied to all the frequency components in the signal. Thus all of these frequencies can only radiate along that one angle and cannot be spread to other directions. Therefore, a phased array can serve users in only one direction at a time and cannot perform flexible directional frequency multiplexing with many users. Split-antenna phased array (Fig. \ref{fig:baseline_architecture_and_heatmap}(b)) uses the same phased array architecture to create multiple beams to serve multiple users in one TTI, but suffers from lower antenna gain, range, and throughput.


\noindent
\textbf{True-time delay array:} The \ttd array uses a delay element to replace the phase shifter as shown in Fig. \ref{fig:baseline_architecture_and_heatmap}(c). The antenna weights with delay element is given by:
% The delay element creates different delays to the input signal at each antenna before they get radiated in space. When multiple copies of these waveforms from each antenna are added at the receiver, they create a unique gain pattern as a function of the frequency content of the signal. To understand it concretely, we define the  antenna weights with delay element as:
\begin{equation}
    w_{\text{delay}}(t,n) = \delta(t-\tau_n)
\end{equation}
% where $\tau_n$ is the variable delay at antenna $n$ and $t$ is the time axis. Upon taking FFT of $\delta(t-\tau_n)$, we get $e^{j2\pi f\tau_n}$. We observe that the phase of this exponential term is frequency-dependent, or in other words, the delay element creates frequency-varying phase at each antenna element. 
% Now how does this enables frequency-selectivity? Unlike traditional phased array which adds a constant phase across all frequencies, we see that here different frequency components experience a different phase shift at each antenna which will make them radiate in different directions. 
% A natural question is whether this delay element can create a desired frequency-selective beams. 
Past work on \ttd array~\cite{yan2019wideband,boljanovic2020true,boljanovic2021fast, li2022rainbow} have shown that this architecture creates a prism-type response by radiating all the frequencies in all the directions in a linear fashion (Fig.~\ref{fig:baseline_architecture_and_heatmap}(c)) by using a fixed set of delays at each antenna given by $\tau_n = \frac{n}{\text{B}}$, for bandwidth $B$. This response has two major limitations: 1) most frequency bands would be wasted in space if there are no user in that direction and 2) each user gets a small frequency band and cannot scale it up arbitrarily. Due to these limitations, \ttd array is not suitable for flexible directional frequency multiplexing.

% \noindent
% \textbf{Delay-phased array:} 


% This phased array consists of a programmable phase shifter at each antenna that modulates the signal with a tunable phase value. This phase modulation enables directed 

% There is a single data input to the phased array which is radiated in space.So, all the frequency bands in the input data is transmitted to the same direction and cannot be separated into different directions. 



% To put it simply, for a phased array with $N$ antennas we can achieve a gain-pattern, $G(\theta)$  by tuning as follows:

% \begin{equation}
%         G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)V(n,\theta)
% \end{equation}
% where the weights at each antenna $w_{\text{phase}}(n)$ consists of  

% $V(n,\theta) = e^{-jn\pi\sin(\theta)}$, is a standard steering matrix transformation from antenna to space-domain\footnote{Note that $V(n,\theta) = e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$ depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$. We assume $d=\frac{\lambda}{2}$ and approximate the array response as $V(n,\theta) = e^{-jn\pi\sin(\theta)}$.}. 

% Further we can easily show that (more details in Appendix~\ref{sec:appendix}.1) $w_{\text{phase}}(n) = e^{jn\pi\sin(\theta_0)}$ are the individual antenna phase that are applied through a programmable phase-shifter at each antenna $n$ as shown in Fig. 3 to beamform towards the desired user direction $\theta_0$. 

% Even if we use multiple phased arrays with multiple inputs from the baseband in a MIMO fashion, each MIMO array might send their data in different directions, but they still can't do frequency multiplexing. Each phased arrays in MIMO would still send the entire input data to one direction. So MIMO arrays are in this way complementary to our problem, they may reduce the number of direction to serve from a single array, but still very resource inefficient because they can't do frequency multiplexing. Fundamentally, we need a way to perform frequency multiplexing with a single antenna array.


% A naive way to serve multiple directions with a single phased array is to divide the array into multiple sub-arrays and program each sub-arrays to radiate in one direction each~\cite{hassanieh2018fast, abari2016millimeter,marjan2018split,aykin2019multi}. In this way the input data can be spread in multiple directions and each user can extract their corresponding frequency bands as shown in Fig.~\ref{fig:phased_array}(c).
% % as shown in Fig.~\ref{fig:conventional_frequency_flat_vs_ours}(a). 
% The issue with this split-antenna approach is that rather than sending one frequency band in one direction and another frequency band in other direction, it sends all the frequency bands to all the directions. As a result, the transmit power is spread at multiple locations in space and so each user gets low power. The mmWave systems loses all the gains due to directional links and severely reduces the throughput and link reliability.


% \subsection{Motivation for \name}


% % \review{R1: The presented motivation for multi-user data transmission is not convincing. Reviewer said no advantage in spectral efficiency.} \todo{Don't say we improve spectral efficiency, but mention that we allow flexible resource allocation and reduce latency.}
% We have seen above how most of the existing mmWave algorithms that phased array compromise on \textcolor{blue}{resource} efficiency and latency due to their inability to perform \textcolor{blue}{flexible frequency multiplexing}. The other split-antenna systems compromise on the net throughput by splitting the antenna arrays.  On the other hand, the \ttd array compromises on throughput to get low latency. Thus it is the need of the hour to develop a system that can perform flexible frequency multiplexing to achieve both high throughput and low latency. It would enable to allocate and transmit only the frequency resources that a user demands in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Fig.~\ref{fig:TDMA_OFDMA_3D}(b)). 
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.

% Therefore, our goal is to selectively radiate in frequency-space axis, and not illuminate all direction for all frequencies as it would reduce range and throughput....\todo{talk about those two scenarios} but we want to localize the beam in both frequency and space dimensions.
% This localization across both frequency and space, only the frequency resources that a user demands are allocated to that user in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Fig.~\ref{fig:TDMA_OFDMA_3D}(b)). 
% In this way, it can support many users with frequency-multiplexing without compromising on directional gains and maintaining high throughput and reliable mmWave links.
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.




\subsection{Current mmWave architectures are incapable for flexible directional frequency multiplexing}
% We compare four analog beamforming architectures for mmWave front-end antenna array and show how they differ in terms of network performance metrics such as latency, effective spectrum usage, and throughput. Those are: 1. phased array, 2. split-antenna array, 3. true-time delay array, and our proposed 4. \dpa; each differ in how they create analog beams towards the users. The architecture details and beampatterns (along both frequency and space dimensions) for all these architectures is shown in Fig.~\ref{fig:baseline_architecture_and_heatmap}. 

Let us take a simple network scenario to understand the performance tradeoffs for the above systems. Consider 100 users in the network with mixed traffic demand: 90 users with 50 Mbps (4K video streaming) and $<8$ms latency demand, and 10 users with 1 Gbps (8k streaming) with $<25$ ms latency demands~\cite{pocovi2018achieving,3gpp2020}. We assume all users are distinctly located and RF conditions are good (e.g. LOS and no blockage), so we truly evaluate on the architecture capabilities itself independent of common external factors. We assume our \dpa and split array create 4 concurrent beams and \ttd array create a prism beam pattern.
The comparison is shown in Table~\ref{tab:compare_baseline_background}. 
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}\hline
        Architecture & Latency & Spectrum usage & Throughput \\\hline
        phased array (TDMA) & 12.5 ms (high) & $\approx5$\% & T units \\\hline
        split-antenna array & 4.1 ms (low) & 100\% & T/4 units\\\hline
        \ttd array & 0 ms & $\approx1$\% & T/10 units \\\hline
        \dpa & 4.1 ms (low) & 100\% & T units\\\hline
    \end{tabular}
    \caption{Comparing \dpa with other architectures.}
    \label{tab:compare_baseline_background}
\end{table}

\todo{please argue that thorughput can be supported for each of these applications, but latency is not good enough...} The phased array performs only time-multiplexing and serve each user in a different time slot and so with protocol specified TTI (transmission-time interval) of 0.125ms~\cite{3gpp2020,pocovi2018achieving,zhang2019machine}. 
Hence, it would take 12.5ms to serve all the 100 users, which would violate the $>8$ms for the 10 users having 8k video requirements. Secondly it leads to significant   spectrum wastage, for example the 90 users from the above scenario are served a 1Gbps link while their requirement is at best for a 50Mbps link, leading to effective spectrum usage as low as $5\%$ \todo{Ish: not convincing numbers, how to improve?}. In contrast, because \dpa can serve 4 directions simultaneously, the latency is reduced by 4x and effective spectrum usage is increased by 4x. Note that TDMA and FDMA ideally provide the same throughput because they use identical number of resource blocks to serve the user. This analysis shows that \name can achieve low latency and better spectrum usage because it allows flexible directional OFDMA (both time and frequency multiplexing with flexibly chosen multiple directional beams).

We also note that Split-antenna array and \ttd array both compromises on throughput to provide low latency. \ttd array is on the other extreme where it can provide extremely low latency (serves all directions in one TTI), but suffers from extremely low data rates. In contrast, our \dpa provides flexibility to perform directional frequency multiplexing with directional pencil beams for all users leading to both high sum throughput and low latency.

% Let us look at how the current mmWave systems have tried to address the increasing demand for data-rates and new users and see where they lack and what are the requirements to overcome these limitations.
% With exponential growth in use of wireless connectivity, a diverse set of applications have emerged. A variety of applications from AR/VR to V2X have a high disparity in their data-rate and latency demands. 
% % On the one hand, there are latency-sensitive applications such as online gaming and vehicular communication, and on the other hand, there are throughput-intensive applications such as VR. 
% For VR applications alone, the data-rate and latency demands vary based on video quality, rendering requirements and resolution ranging from 20 Mbps at 40fps for a simple 4k VR video streaming to 400fps at 1 Gbps for 8k on-headset tethered VR.
% % It is envisioned that the high-frequency mmWave bands could support these high-throughput and frame-rate demanding applications with a large amount of spectrum available at these frequencies. Furthermore, today's mmWave deployment is mostly limited to being able to serve one user at a time slot, and then multiplex over time-slots to serve multiple users. 
% % In each slot direction of the one user who is going to be served is illuminated by the mmWave beams. 

% % There are two problems with this approach. First, the users must wait for their turn to be served, which causes large delays for high-throughput and high-frame rate applications like tethered VR.
% % For instance, let us consider 
% Consider an example where a base station is serving 100 different VR users, in a 10-90 split, where the 10 users are tethering 8k VR streams on headsets and need a 1Gbps link with $<8$msec latency requirements, while the rest 90 users are streaming 4k VR videos requiring 50Mbps links with $<25$msec latency.
% Since, existing mmWave can only perform time-multiplexing, they have to serve each of the user in a different time slot, with protocol specified TTI (transmission-time interval) of 0.125msec \cite{pocovi2018achieving,zhang2019machine}. 
% Hence, it would take 12.5ms to serve all the 100 users, which would violate the $>8$msec for the 10 users having 8k video requirements. 
% % to serve the Gbps users the next frame leading to lags and frame drops.
% % \todo{reads odd, use "significant" instead of very}
% Secondly it leads to significant   spectrum wastage, for example the 90 users from the above scenario are served a 1Gbps link while their requirement is at best for a 50Mbps link, leading to spectral efficiencies as low as $5\%$.
% Thus scaling up the current mmWave systems to multiple users for these targeted applications is not possible, as they cannot meet the latency requirements for the high throughput demanding VR applications and are highly inefficient in spectral resource utilization.

% For instance, a base station with a narrow $6^\circ$ beam would scan $360^\circ/6^\circ = 60$ directions in azimuth angle and roughly 4x more to cover the elevation angles. This large angular diversity may cause up to 100 ms delay, which is intolerable for applications such as online gaming, which requires 10-20 ms end-end latency. Secondly, due to disparity in user demands, some applications require as low as 20 Mbps. Still, the base station allocates the entire bandwidth (a multi Gbps connection) resource to this user leading to the wastage of precious spectrum resources.
% We take insights from sub-6 communication, which efficiently serves multiple users with flexible time-frequency multiplexing. Therefore, it is logical to extend these capabilities for mmWave links too to enable efficient multi-user communication.

% Current millimeter-wave system can't perform flexible frequency multiplexing because they use an antenna array to beamform signal to a specific direction and can only serve that direction. Though a fully-digital beamforming architecture can create frequency-selective beams, they are not feasible for mmWave bands because of high power and complexity in laying hundreds of RF chains for each antenna element.
% The sub-6 systems can easily do frequency multiplexing because it uses an omnidirectional antenna to radiate in all directions and so the intended users can receive data in their assigned frequency band and discard data in other bands. When the gNB has multiple antennas in MIMO-OFDMA system, it is possible to digitally beamform different frequency bands to different users. But, mmWave MIMO system is impractical because of high power and complexity in laying hundreds of RF chains for each antenna element. 

% In contrast, mmWave front-end consists of analog antenna array for beamforming. Three common analog array architectures are: phased array, split-antenna array and true-time delay array. Here we show how these three architectures fail to perform flexible frequency multiplexing and suffer from either low throughput or high latency when serving multiple users in the network as shown in Fig.~\ref{fig:compare_baselines_motivation}. The phased array provide high throughput when there are only few high-traffic users, but fails in a mixed or low traffic scenarios. It wastes a lot of spectrum and suffers from low throughput and high latency. Split-antenna array compromises on throughput to provide low latency. Finally, \ttd array is on the other extreme where it can provide low latency for sensitive IoT applications, but suffers from extremely low data rates. In contrast, our \dpa provides flexibility to perform frequency multiplexing with highly directional pencil beams for all users leading to both high sum throughput and low latency.





==> Arxiv/2_motivation_v3.tex <==
% !TEX root = main.tex
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/baseline_architecture_and_heatmap.pdf}
    \caption{Comparison of different mmWave front-end architectures and corresponding frequency-space patterns they created. The traditional phased array and split-antenna array create a frequency-flat response, while \ttd array creates a frequency-selective rainbow-like pattern radiating in all directions. In contrast, \dpa provides flexibility to create arbitrary frequency-direction response. 
    % Note all frequency-space heatmaps are simulated with 8 antenna arrays and plotted with the same x-axis (angle from $-90^\circ$ to $90^\circ$), y-axis (frequency from -200 MHz to 200 MHz), and colorbar (Antenna gain from 0 to 5 dB). 
    }
    \label{fig:baseline_architecture_and_heatmap}
\end{figure*}

\section{Background and Motivation}\label{sec:motivation}
% More in Infocom v2: Reverse primer and example.
% # New in Infocom v2: Provide short comparison with 3 baselines in table form. 
% New in v3: improve 3.2 first by removing all the maths and explain intuitively and then work in simplifying 3.1
% v4: Completely new way to put this section based on Dinesh's feedback. 2.1 Applications, resource inefficiency. 2.2 Sub-6 OFDMA is great but not possible with mmWave - hybrid, splitantenna baseline etc. 2.3 Our insight/motivation without giving delay architecture. Tell why you need it and not how you use it.

In this section, we would provide a primer on different analog antenna array architectures, which have a single baseband radio frequency (RF) chain and mechanism to best achieve flexibility in resource allocation to multiple users. Next, we would show a realistic example that none of the architecture can meet the requirements for flexible directional frequency multiplexing, and how our flexible \dpa architecture can meet these requirements. 


\subsection{Primer on phased arrays and true-time delay arrays}
\textbf{$\blacksquare$ Phased array:}
The phased array takes a single input from the digital chain, split into $N$ copies, phase-shifted and radiated from $N$ antennas (Fig. \ref{fig:baseline_architecture_and_heatmap}(a)). The input signal consisting of all frequency bands is radiated in space with a beam pattern given by:
% One of the reasons why current mmWave technology cannot achieve better quality of service is due to its inability to serve multiple users with flexible time-frequency multiplexing.
% Efficient frequency multiplexing is a viable way to serve multiple users in a resource efficient manner as only required set of frequency resources can be allocated to users along different directions without compromising the link quality in any given direction.
% However current mmWave technology cannot perform frequency multiplexing due to an inflexible analog front-end architecture. The mmWave front-end uses a phased array architecture connected to the baseband with a single wire interface as shown in Fig.~\ref{fig:phased_array}. This phased array takes the input signal from baseband and radiates it into space. 
% While radiating the signal, each individual antenna has a phase-shifter that adds an additional phase shift to the signal.
% These additional phase shifts at each antenna combine the signal such that one fixed angle gets the highest antenna gain while severely suffering at other angles. This directional gain is enabled to provide reliable throughput link to the user by overcoming the high attenuation rates of mmWave signals.
% To put it simply, the gain pattern of a phased array with $N$ antennas is given by:
% \begin{equation}\label{eq:phasedarraygain}
%         G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)e^{-jn\pi\sin(\theta)}
% \end{equation}
% where the weights 
\begin{equation}
    w_{\text{phase}}(n) = e^{j\Phi_n}
\end{equation}
contains programmable phases $\Phi_n$ for antenna index $n (n\in [0,N-1])$ and   $e^{-jn\pi\sin(\theta)}$ is the standard steering vector transformation from antenna to space ($\sin(\theta)$)-domain\footnote{Note that the steering vector for a linear antenna array is given by  $e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$, which depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$~\cite{benesty2019array}. We assume $d=\frac{\lambda}{2}$ and approximate the steering vector as $e^{-jn\pi\sin(\theta)}$.}. Now, if we program the phases to create a directional beam at an angle say $\theta_0$, then all the same phase offset is applied to all the frequency components in the signal. Thus all of these frequencies can only radiate along that one angle and cannot be spread to other directions. Therefore, a phased array can serve users in only one direction at a time and cannot perform flexible directional frequency multiplexing with many users. Split-antenna phased array (Fig. \ref{fig:baseline_architecture_and_heatmap}(b)) uses the same phased array architecture to create multiple beams to serve multiple users in one TTI, but suffers from lower antenna gain, range, and throughput.


\noindent
\textbf{$\blacksquare$ True-time delay array:} The true-time delay (\ttd) array uses a delay element to replace the phase shifter as shown in Fig. \ref{fig:baseline_architecture_and_heatmap}(c). The antenna weights with delay element is given by:
% The delay element creates different delays to the input signal at each antenna before they get radiated in space. When multiple copies of these waveforms from each antenna are added at the receiver, they create a unique gain pattern as a function of the frequency content of the signal. To understand it concretely, we define the  antenna weights with delay element as:
\begin{equation}
    w_{\text{delay}}(t,n) = \delta(t-\tau_n)
\end{equation}
% where $\tau_n$ is the variable delay at antenna $n$ and $t$ is the time axis. Upon taking FFT of $\delta(t-\tau_n)$, we get $e^{j2\pi f\tau_n}$. We observe that the phase of this exponential term is frequency-dependent, or in other words, the delay element creates frequency-varying phase at each antenna element. 
% Now how does this enables frequency-selectivity? Unlike traditional phased array which adds a constant phase across all frequencies, we see that here different frequency components experience a different phase shift at each antenna which will make them radiate in different directions. 
% A natural question is whether this delay element can create a desired frequency-selective beams. 
Past work on \ttd array~\cite{yan2019wideband,boljanovic2020true,boljanovic2021fast, li2022rainbow} have shown that this architecture creates a prism-type response by radiating all the frequencies in all the directions in a linear fashion (Fig.~\ref{fig:baseline_architecture_and_heatmap}(c)) by using a fixed set of delays at each antenna given by $\tau_n = \frac{n}{\text{B}}$, for bandwidth $B$. This response has two major limitations: 1) most frequency bands would be wasted in space if there are no user in that direction and 2) each user gets a small frequency band and cannot scale it up arbitrarily. Due to these limitations, \ttd array is not suitable for flexible directional frequency multiplexing.

% \noindent
% \textbf{Delay-phased array:} 


% This phased array consists of a programmable phase shifter at each antenna that modulates the signal with a tunable phase value. This phase modulation enables directed 

% There is a single data input to the phased array which is radiated in space.So, all the frequency bands in the input data is transmitted to the same direction and cannot be separated into different directions. 



% To put it simply, for a phased array with $N$ antennas we can achieve a gain-pattern, $G(\theta)$  by tuning as follows:

% \begin{equation}
%         G(\theta) = \sum_{n=0}^{N-1}w_{\text{phase}}(n)V(n,\theta)
% \end{equation}
% where the weights at each antenna $w_{\text{phase}}(n)$ consists of  

% $V(n,\theta) = e^{-jn\pi\sin(\theta)}$, is a standard steering matrix transformation from antenna to space-domain\footnote{Note that $V(n,\theta) = e^{-jn2\pi \frac{d}{\lambda} \sin(\theta)}$ depends on the array geometry (antenna spacing $d$) and signal wavelength $\lambda$. We assume $d=\frac{\lambda}{2}$ and approximate the array response as $V(n,\theta) = e^{-jn\pi\sin(\theta)}$.}. 

% Further we can easily show that (more details in Appendix~\ref{sec:appendix}.1) $w_{\text{phase}}(n) = e^{jn\pi\sin(\theta_0)}$ are the individual antenna phase that are applied through a programmable phase-shifter at each antenna $n$ as shown in Fig. 3 to beamform towards the desired user direction $\theta_0$. 

% Even if we use multiple phased arrays with multiple inputs from the baseband in a MIMO fashion, each MIMO array might send their data in different directions, but they still can't do frequency multiplexing. Each phased arrays in MIMO would still send the entire input data to one direction. So MIMO arrays are in this way complementary to our problem, they may reduce the number of direction to serve from a single array, but still very resource inefficient because they can't do frequency multiplexing. Fundamentally, we need a way to perform frequency multiplexing with a single antenna array.


% A naive way to serve multiple directions with a single phased array is to divide the array into multiple sub-arrays and program each sub-arrays to radiate in one direction each~\cite{hassanieh2018fast, abari2016millimeter,marjan2018split,aykin2019multi}. In this way the input data can be spread in multiple directions and each user can extract their corresponding frequency bands as shown in Fig.~\ref{fig:phased_array}(c).
% % as shown in Fig.~\ref{fig:conventional_frequency_flat_vs_ours}(a). 
% The issue with this split-antenna approach is that rather than sending one frequency band in one direction and another frequency band in other direction, it sends all the frequency bands to all the directions. As a result, the transmit power is spread at multiple locations in space and so each user gets low power. The mmWave systems loses all the gains due to directional links and severely reduces the throughput and link reliability.


% \subsection{Motivation for \name}


% % \review{R1: The presented motivation for multi-user data transmission is not convincing. Reviewer said no advantage in spectral efficiency.} \todo{Don't say we improve spectral efficiency, but mention that we allow flexible resource allocation and reduce latency.}
% We have seen above how most of the existing mmWave algorithms that phased array compromise on \textcolor{blue}{resource} efficiency and latency due to their inability to perform \textcolor{blue}{flexible frequency multiplexing}. The other split-antenna systems compromise on the net throughput by splitting the antenna arrays.  On the other hand, the \ttd array compromises on throughput to get low latency. Thus it is the need of the hour to develop a system that can perform flexible frequency multiplexing to achieve both high throughput and low latency. It would enable to allocate and transmit only the frequency resources that a user demands in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Fig.~\ref{fig:TDMA_OFDMA_3D}(b)). 
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.

% Therefore, our goal is to selectively radiate in frequency-space axis, and not illuminate all direction for all frequencies as it would reduce range and throughput....\todo{talk about those two scenarios} but we want to localize the beam in both frequency and space dimensions.
% This localization across both frequency and space, only the frequency resources that a user demands are allocated to that user in one direction and the rest of the resources can be allocated to another directional user without getting wasted (See Fig.~\ref{fig:TDMA_OFDMA_3D}(b)). 
% In this way, it can support many users with frequency-multiplexing without compromising on directional gains and maintaining high throughput and reliable mmWave links.
% To that extent we have developed \name, by enabling frequency-multiplexing with a single mmWave antenna array. We will discuss in next section how we create frequency-selective beams to enable this frequency multiplexing.

\subsection{Current mmWave architectures are incapable for flexible directional frequency multiplexing}
% We compare four analog beamforming architectures for mmWave front-end antenna array and show how they differ in terms of network performance metrics such as latency, effective spectrum usage, and throughput. Those are: 1. phased array, 2. split-antenna array, 3. true-time delay array, and our proposed 4. \dpa; each differ in how they create analog beams towards the users. The architecture details and beampatterns (along both frequency and space dimensions) for all these architectures is shown in Fig.~\ref{fig:baseline_architecture_and_heatmap}. 

Let us take a simple network scenario to understand the performance tradeoffs for the above systems. Typically for 4K VR applications, end-end latency should be $< 100$ ms, Where transmission goes from the public cloud, network provider, base station (edge), and device. Over-the-air (base station to device) transmission latency comes down to a strict latency requirement of $< 1$ ms \cite{qualcomm2017augmented}. Consider 10 users in the network with similar traffic demand: each user requires 60 Mbps (4K VR) throughput and $<1$ ms over-the-air latency due to the interactive nature of VR~\cite{pocovi2018achieving,3gpp2020,qualcomm2017augmented,mangiante2017vr}. The aggregate throughput provided by the users is 600 Mbps, only 30\% of the max physical layer throughput of a 400 MHz FR2 gNB in downlink (2.2 Gbps). We assume all users are distinctly located (in different angular directions) and RF conditions are good (e.g. LOS and no blockage). This allows us to control common external factors and exclusively evaluate architectural capabilities. We assume our \dpa and split array can create up to 8 concurrent beams and \ttd array creates a prism beam pattern. The comparison is shown in Table~\ref{tab:compare_baseline_background}. From our end-end evaluations (Fig.~\ref{fig:latency_only}), we can see that in edge scenarios all the baselines failed to meet the $1 $ ms over-the-air latency requirement. It is evident that \name is the best to support latency-critical applications while satisfying higher throughput demands.
\begin{table}[h]
    \centering
    \footnotesize
    \begin{tabular}{|c|c|c|c|}\hline
        Architecture & Latency* (ms) & Packet Loss & Throughput \\\hline
        phased array (TDMA) & $> 1.25$ ms & 24.0\% & 54.9 Mbps \\\hline
        split-antenna array & $> 2$ ms  & 33.3\% & 47.3 Mbps \\\hline
        \ttd array & $> 3.5 $ ms & 76.4\% & 18.3 Mbps \\\hline
        \dpa & $< 0.5$ ms & 0.0\% & 71.3 Mbps\\\hline
    \end{tabular}
    \caption{Delay-phased array \& other baselines for 10 4k VR users (*We mention over-the-air worst case latency).}
    \label{tab:compare_baseline_background}
\end{table}

% Due to the low traffic demand per user and the multiple user directions, scheduling data to the users under throughput and latency constraints becomes difficult. The phased array performs only time-multiplexing and serves each user in a different time slot, we observed that worst-case latency is more than 1.25 ms. Hence, it violates the latency constraint of $<1$ ms for some of the users. Latency constraint violations lead to dropped packets and result in poor user experience. In contrast, because \dpa can serve 8 directions simultaneously, it can pack user data more effectively, which is less than 0.2 ms for all scenarios. This analysis shows that \name can achieve low latency and better spectrum usage because it allows flexible directional OFDMA.
% (both time and frequency multiplexing with flexibly chosen multiple directional beams).
%
% We also note that the Split-antenna array and \ttd array both compromises on throughput to provide low latency. \ttd array is on the other extreme where it can provide extremely low latency (serves all directions in one TTI) but suffers from extremely low data rates. 
%
% We also note that the Split-antenna array and \ttd array with low data rates lead to incomplete packet deliveries and ultimately lead to packet loss. In contrast, our \dpa provides flexibility to perform directional frequency multiplexing with directional pencil beams for all users leading to both high sum throughput and low latency. The setup and results of Table~\ref{tab:compare_baseline_background} are detailed in Sec.~\ref{sec:evaluation}.

% Let us look at how the current mmWave systems have tried to address the increasing demand for data-rates and new users and see where they lack and what are the requirements to overcome these limitations.
% With exponential growth in use of wireless connectivity, a diverse set of applications have emerged. A variety of applications from AR/VR to V2X have a high disparity in their data-rate and latency demands. 
% % On the one hand, there are latency-sensitive applications such as online gaming and vehicular communication, and on the other hand, there are throughput-intensive applications such as VR. 
% For VR applications alone, the data-rate and latency demands vary based on video quality, rendering requirements and resolution ranging from 20 Mbps at 40fps for a simple 4k VR video streaming to 400fps at 1 Gbps for 8k on-headset tethered VR.
% % It is envisioned that the high-frequency mmWave bands could support these high-throughput and frame-rate demanding applications with a large amount of spectrum available at these frequencies. Furthermore, today's mmWave deployment is mostly limited to being able to serve one user at a time slot, and then multiplex over time-slots to serve multiple users. 
% % In each slot direction of the one user who is going to be served is illuminated by the mmWave beams. 

% % There are two problems with this approach. First, the users must wait for their turn to be served, which causes large delays for high-throughput and high-frame rate applications like tethered VR.
% % For instance, let us consider 
% Consider an example where a base station is serving 100 different VR users, in a 10-90 split, where the 10 users are tethering 8k VR streams on headsets and need a 1Gbps link with $<8$msec latency requirements, while the rest 90 users are streaming 4k VR videos requiring 50Mbps links with $<25$msec latency.
% Since, existing mmWave can only perform time-multiplexing, they have to serve each of the user in a different time slot, with protocol specified TTI (transmission-time interval) of 0.125msec \cite{pocovi2018achieving,zhang2019machine}. 
% Hence, it would take 12.5ms to serve all the 100 users, which would violate the $>8$msec for the 10 users having 8k video requirements. 
% % to serve the Gbps users the next frame leading to lags and frame drops.
% % \todo{reads odd, use "significant" instead of very}
% Secondly it leads to significant   spectrum wastage, for example the 90 users from the above scenario are served a 1Gbps link while their requirement is at best for a 50Mbps link, leading to spectral efficiencies as low as $5\%$.
% Thus scaling up the current mmWave systems to multiple users for these targeted applications is not possible, as they cannot meet the latency requirements for the high throughput demanding VR applications and are highly inefficient in spectral resource utilization.

% For instance, a base station with a narrow $6^\circ$ beam would scan $360^\circ/6^\circ = 60$ directions in azimuth angle and roughly 4x more to cover the elevation angles. This large angular diversity may cause up to 100 ms delay, which is intolerable for applications such as online gaming, which requires 10-20 ms end-end latency. Secondly, due to disparity in user demands, some applications require as low as 20 Mbps. Still, the base station allocates the entire bandwidth (a multi Gbps connection) resource to this user leading to the wastage of precious spectrum resources.
% We take insights from sub-6 communication, which efficiently serves multiple users with flexible time-frequency multiplexing. Therefore, it is logical to extend these capabilities for mmWave links too to enable efficient multi-user communication.

% Current millimeter-wave system can't perform flexible frequency multiplexing because they use an antenna array to beamform signal to a specific direction and can only serve that direction. Though a fully-digital beamforming architecture can create frequency-selective beams, they are not feasible for mmWave bands because of high power and complexity in laying hundreds of RF chains for each antenna element.
% The sub-6 systems can easily do frequency multiplexing because it uses an omnidirectional antenna to radiate in all directions and so the intended users can receive data in their assigned frequency band and discard data in other bands. When the gNB has multiple antennas in MIMO-OFDMA system, it is possible to digitally beamform different frequency bands to different users. But, mmWave MIMO system is impractical because of high power and complexity in laying hundreds of RF chains for each antenna element. 

% In contrast, mmWave front-end consists of analog antenna array for beamforming. Three common analog array architectures are: phased array, split-antenna array and true-time delay array. Here we show how these three architectures fail to perform flexible frequency multiplexing and suffer from either low throughput or high latency when serving multiple users in the network as shown in Fig.~\ref{fig:compare_baselines_motivation}. The phased array provide high throughput when there are only few high-traffic users, but fails in a mixed or low traffic scenarios. It wastes a lot of spectrum and suffers from low throughput and high latency. Split-antenna array compromises on throughput to provide low latency. Finally, \ttd array is on the other extreme where it can provide low latency for sensitive IoT applications, but suffers from extremely low data rates. In contrast, our \dpa provides flexibility to perform frequency multiplexing with highly directional pencil beams for all users leading to both high sum throughput and low latency.





==> Arxiv/3_design.tex <==
% !TEX root = main.tex
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fsda_explain.pdf}
    \caption{Explanation on how \dpa creates a desired frequency-space image in (a) with two beams at $0^\circ$ and $30^\circ$. The $0^\circ$ beam occupies frequency range in [-200,0] MHz and $30^\circ$ beam occupies frequency range of [0,200] MHz. Specific frequency-space signatures are shown in (b) and (c) with antenna sub-arrays and final frequency-space image is shown in (d) and (e) with 4 and 8 antennas respectively.}
    \label{fig:fsda_explain}
\end{figure*}

\section{Design of \name} \label{sec:design}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/delay_per_antenna_fig.pdf}
%     \caption{Shows our proposed mmWave system which implements variable delays and phases per-antenna to create frequency-selective beams.}
%     \label{fig:delay_per_antenna_fig}
% \end{figure}

 \begin{figure} [!t]
    \subfigure{{\includegraphics[width=0.23\textwidth]{figures/design_delay_range_vs_UEs.pdf}\label{fig:user_variations}}}
    \subfigure{{\includegraphics[width=0.23\textwidth]{figures/design_delay_range_vs_antennas.pdf}\label{fig:antenna_variations}}}
    % \subfigure{{\includegraphics[width=0.24\textwidth]{figures/benchmark_convergence.pdf}\label{fig:convergence}}}
    \caption{Delay range for \name's \dpa with (a) Number of splits/user directions and (b) Number of antennas. Shows average and standard deviation of multiple random trials, each with random set of angles and frequency bands for specific number of user directions. }
    % \vspace{4pt}
 \end{figure}

% \review{R2 and R1: It is not clear to me how you can transmit multiple streams to multiple users using a single-chain. Since the delays are only introducing phases, how do we generate different data streams to different users? I am assuming that you have to use multiple chains so as to rtansmit different data streams to different users. If this is the case, would this not be the largest source of complexity in this architecture? why not use M chains each with its own phase array front end and coordinate between the chains in software? Wouldn't that be simpler? I think comparing with these different architectures would be important to understand if the benefits of this work are really validated.} \todo{Explicitly mention "flexible frequency multiplexing" often}.
\name designs a new mmWave front-end architecture called \dpa to enable flexible directional frequency multiplexing for mmWave network. 
We have seen in ~\cref{sec:motivation} how the existing mmWave phased array and \ttd array fail to create the desired frequency-direction response. In section~\cref{sec:design-dpa}, we describe how we create such a response with \dpa. We then describe the range and resolution analysis for the delay element in \dpa in ~\cref{sec:design-range} and present our novel algorithm to estimate optimal delays and phases in~\cref{sec:design-est}.  
% Finally, we evaluate \name with a real-time scheduler, traffic generator and \dpa emulation in ~\cref{sec:evaluation} and conclude the paper with a discussion on practical aspects of \dpa.
% We then describe how the new programmable front-end integrates with higher layers in the networking stack in ~\cref{sec:design-real}. 
% We specifically focus on our scheduler design logic which determines which users to serve in each time-slot and over what frequency bands and show the end-to-end system of \name.
% Finally, we conclude by addressing important system-level challenges in building end-to-end system with \name in ~\cref{sec:design-real}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/range_requirement_ttd_vs_dpa.pdf}
%     \caption{\textcolor{blue}{In contrast to true-time delay arrays, our \dpa has lenient delay range requirements which is better feasible to implement in circuits~\cite{ghaderi2019integrated}.}}
%     \label{fig:range_requirement_ttd_vs_dpa}
% \end{figure}

\subsection{How delay-phased array creates arbitrary frequency-direction beam response?}\label{sec:design-dpa}


% Before we explain how \dpa works, we first focus on the delay element and show how it enables frequency-selectivity. The delay element creates different delays to the input signal at each antenna before they get radiated in space. When multiple copies of these waveforms from each antenna are added at the receiver, they create a unique gain pattern depending on the frequency content of the signal. To understand it concretely, we define the  antenna weights with delay element as:
% \begin{equation}
%     w_{\text{phase}}(t,n) = \delta(t-\tau_n)
% \end{equation}
% where $\tau_n$ is the variable delay at antenna $n$ and $t$ is the time axis. 

% Here we can intuitively understand that a time varying signal has a certain frequency response. Upon taking FFT of $\delta(t-\tau_n)$, we get $e^{j2\pi f\tau_n}$. We observe that the phase of this exponential term is frequency-dependent, or in other words, the delay element creates frequency-varying phase at each antenna element. Now how does this enables frequency-selectivity? Unlike traditional phased array which adds a constant phase across all frequencies, we see that here different frequency components experience a different phase shift at each antenna which will make them radiate in different directions. 

% A natural question is whether this delay element can create a desired frequency-selective beams. Past work on delay-only array\footnote{Delay-only array is referred as true-time delay array in literature.}~\cite{yan2019wideband, boljanovic2020design,wadaskar20213d,boljanovic2020true,boljanovic2021fast} have shown that this architecture creates a prism-type response by radiating all the frequencies in all the directions in a linear fashion as shown in Fig.~\ref{fig:delay_per_antenna_fig}(b). This response has two major limitations: 1) most frequency bands would be wasted in space if there are no user in that direction and 2) each user gets a small frequency band and cannot scale it up arbitrarily. Due to these limitations, delay-only array is not suitable for our multi-user communication scenario. 

% In \name, for the first time, we show that any arbitrary frequency-space response is achievable with appropriate programming of \dpa. 
% The \dpa architecture consists of a variable delay and a variable phase element at each antenna as shown in Fig.~\ref{fig:baseline_architecture_and_heatmap}(d). So far we have seen that the phase element alone cannot achieve frequency-selectivity and the delay element alone cannot create arbitrary and controlled frequency-selective beams. 

Our goal is to construct arbitrary frequency-direction mapping ($G(f,\theta)$ via an analog antenna array architecture, which would be energy efficient and enable efficient resource utilization and low latency. If we carefully notice example in section 2, we observe that the split antenna achieve the frequency-direction mapping but with a loss of 6 dB SNR, which is a corollary of the entire 400 MHz radiated in each of the four directions. It leads to our first requirement:   
\noindent
\textbf{Req.1:} \textit{The signal must be transmitted/received in frequency-direction used by users, i.e.  each band of frequencies must be radiated only in the direction of users they are associated with, and frequencies not associated with the user-direction must have no energy  i.e., create a null at those frequencies}
Furthermore, we should be able to control amount of bandwidth assigned to each user, which leads to: 
\noindent
\textbf{Req.2:} \textit{Creating beams narrow in space (for higher antenna gain) but arbitrarily wide in frequency domain (to support high demand users):}



Our \dpa consists of delay and phase elements (Fig.~\ref{fig:baseline_architecture_and_heatmap}(d)). Thus the antenna weights have contribution from these two elements:
\begin{equation}
    w_{\text{dpa}}(t,n) = w_{\text{phase}}(n)w_{\text{delay}}(t,n)= e^{j\Phi_n}\delta(t-\tau_n)
\end{equation}
The gain pattern with \dpa is a function of frequency and space ($\sin(\theta)$) as:
\begin{equation}\label{eq:gain}
    G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) w_\text{dpa}(k,n) V(n,\theta)
\end{equation}
% \begin{equation}\label{eq:gain}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% \end{equation}
% $w_{\text{dpa}}(k,n) = \delta(kT_s-\tau_n)e^{j\Phi_n}$ is the antenna weights, 
where $\Ubf(f,k)$ is a discrete domain Fourier transform (DFT) and the steering matrix $V(n,\theta)$ is explained before in (\ref{eq:phasedarraygain}). Now since the signal is actually sampled only discretely with a sampling time of $T_s$, our original delay weight element $w_{\text{delay}}(t,n)$ would reduce to $w_{\text{delay}}(k,n) = \delta(kT_s-\tau_n)$ as described in (\ref{eq:gain}).

Our insight is to control two knobs: delays $\tau_n$ and phase $\Phi_n$ to get the desired response. 
By taking FFT and equating exponential phase to that of array response, we get: $\Phi_n + 2\pi f \tau_n = n\pi \sin(\theta)$. The variable-delay causes a slope in frequency ($f$) - space ($\sin \theta$) plot, while the variable-phase causes a constant shift along the space axis. Together, they can create an arbitrary line with configurable slope and intercept in frequency-space domain. We delineate two requirements to create desired frequency-direction beam response:





% We set two \textbf{requirements} for achieving such response: 1) The frequency bands must be transmitted along the user directions and not along other directions where there is no user, i.e., create a null in those directions. 2) Provide a large chunk of frequency bands to each user with narrow beams. We take insights from both both delay-domain and phase-domain to meet these requirements. Basically, delay and phase are two knobs in \dpa and by appropriately tuning these two knobs, we could achieve our desired response. 


% Let's understand it through a simple example with two distinctly located users where we stream half frequency bands to one user and another half to other user. Here the desired frequency-space image will look like shown in Fig.~\ref{fig:delay_per_antenna_fig}(d). How should we set the delays and phases to achieve this response? For simplicity, lets first consider only two antennas with relative delay $\Delta\tau$ and relative phase $\Delta\Phi$. Our main insight is that the delay causes a slope in frequency-space domain, while the phase causes a constant shift in space domain. Together, they can create an arbitrary line with configurable slope and intercept in frequency-space domain.



We explain how we achieve these requirements through a simple two user example in Fig.~\ref{fig:fsda_explain}. Let us consider the two users are located at $0^\circ$ and $30^\circ$ respectively and the base station wishes to serve these two users over two different frequency bands in a single timeslot. To support such flexible directional frequency multiplexing, the base station must create a frequency-direction beam response shown in Fig.~\ref{fig:fsda_explain}(a). For simplicity, we call such 2D beam patterns as \textit{frequency-space images}. So how does \dpa create these images and meet the requirements laid above? 



% Let us take a simple example how we create a desired frequency-space image in Fig.~\ref{fig:fsda_explain}(d) with two distinctly located users where we stream half frequency bands to one user and another half to other user. We define two requirements for creating such response as follows:
We achieve these requirements by assigning two antenna sub-arrays of the given antenna array to create complementary response as shown in Fig.~\ref{fig:fsda_explain}(b) and (c) respectively. We see that the first sub-array uses first three antennas to creates a frequency-space image with a positive slope, while the second sub-array create negative slope. Note the two slopes in Fig.~\ref{fig:fsda_explain}(c) is due to aliasing. It happens when relative delay between antenna is larger than $\frac{1}{B}$~\cite{li2022rainbow} and is akin to aliasing due to $d>\frac{\lambda}{2}$ in standard phased arrays~\cite{benesty2019array}. 
% \footnote{Fig.~\ref{fig:fsda_explain}(b) shown two slopes in frequency-space image which can be explained by aliasing feature in phased array. Interested readers are directed to~\cite{benesty2019array} for more details on aliasing}. 
When the two responses are combined together we observe a frequency-space image in Fig.~\ref{fig:fsda_explain}(d) that they combine constructively at desired user locations while create a null (low gain) at other locations (Meeting \textbf{Req-1}). 

For the second requirement, we create such beams by choosing the number of antennas in each sub-arrays. More antenna in a sub-array makes the corresponding signature image narrow in space. For instance, it is easy to visualize from Fig.~\ref{fig:fsda_explain}(b) and (c) that the former response is narrow in space (obtained with 3 antennas) and the later is wider in space (obtained with 2 antennas). In fact, if we have more antennas, say 8 of them, then we can get even `sharper' response as shown in Fig.~\ref{fig:fsda_explain}(e) due to higher constructive combining gains. So, in summary, by controlling the variable-phases and variable-delay knobs of different sub-arrays and the number of antennas in each sub-arrays, we could achieve an arbitrary frequency-space image. 

This intuition helps in understanding how fundamentally any frequency-space image can be created, but it does not help yet on what values of delays and phases we should apply at each antenna to create this image or rather how to estimate these values of delays and phases accurately in real-time. We develop a novel algorithm to estimate delays and phases in real-time in section \ref{sec:design-est}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/algo_fsda_steps.pdf}
    \caption{Three steps of our \algoname algorithm to estimate per-antenna delays and phases that generate a desired frequency-space image. The core step is our novel 2D FSDA transform with some pre-processing and post-processing of inputs and outputs respectively. }
    \label{fig:algo_fsda_steps}
\end{figure*}




\subsection{Variable-Delay's Range and Resolution}\label{sec:design-range}
Before moving to real-time tuning, one final piece of puzzle with \dpa architecture is to determine what ranges of delays the hardware must support to create desired frequency-direction response. The variable-delay's range depends on the system bandwidth and the array field-of-view, i.e., the maximum angular range of the array. The choice of variable-delay per-antenna, for a given bandwidth, and angular FoV can be obtained by equating the antenna phase to the phase of steering vector as: $2\pi f \tau = \pi\sin(\theta)$. This gives, the range of $\tau = \frac{\pi}{2\pi 400e6}=1.25 ns$ per-element for 400 MHz bandwidth and angular range of 90$^\circ$, i.e. the maximum relative delay between any two antenna element is $1.25$ ns. 

% \textcolor{blue}{
The total range of delays depends on the number of antennas and the number of concurrent beams created by the \dpa. To understand this relationship, we performed empirical evaluation with varying number of user directions and antennas in Fig.~\ref{fig:user_variations}, and \ref{fig:antenna_variations} respectively. We observe that \name's \dpa has a lenient requirement on the range of delay values. For instance, the range of delay for \ttd array is $1.25(N-1) ns = 18.75 ns$ for $N = 16$ elements in a uniform linear array~\cite{yan2019wideband, boljanovic2020design,boljanovic2020true,boljanovic2021fast} which increases linearly with number of antennas. Such large delay values are hard to create in circuits due to high losses in transmission lines~\cite{ghaderi2019integrated}.  

In contrast, the delay range in \dpa becomes independent of $N$ when $N$ is large, as shown in Fig. \ref{fig:antenna_variations}. For instance, with $N=16$ antenna or higher and four simultaneous beams, \dpa requires a range of $8.75$ns, which is smaller than true-time delay arrays. The reason why we require less delay range comes from our Requirement-1 of creating nulls in frequency-space images. The null is created using a large negative relative delay (to create beams with negative slope and aliasing in the second sub-array as shown in Fig.~\ref{fig:fsda_explain}(c)), which resets the continuously increasing delay of the first sub-array. Thus, the \dpa range is lower than that of true-time delay arrays, which do not create any nulls.
% as shown in Fig.~\ref{fig:range_requirement_ttd_vs_dpa}.
% }


Similarly, we can obtain the resolution in the variable-delay's values that represents the minimum step-size in delay variation the hardware should support. The delay resolution is obtained as $\frac{0.2\pi}{2\pi 400e6} = 0.25$ns for the beam width of $\sin(12^\circ)=0.2$. 

In summary, the \dpa must provide a range of 8.75 ns with the step-size of 0.25 ns for the variable-delay element. These delays can be implemented in the IF stage of the phased array, with the required resolution and minimal power loss. Delays with sub-ns control have been demonstrated for full-duplex wireless applications~\cite{nagulu2021full,mondal20172,garakoui2015compact} which use the delay effect to mimic the self-interference channel. Recently,~\cite{boljanovic2021fast,park201315,ma2015silicon,ghaderi2020four} have combined accurate delay elements with arrays in commercial grade RFICs. Additionally, in~\cite{ghaderi2020four}, the authors develop a 0.1 ns resolution delay element with 6 bits of range control, well within the requirements of our system. In \name, we propose to repurpose these delays to create the desired frequency-direction response for flexible directional frequency multiplexed mmWave communications.


% delay in IF and 1. How practical phased arrays reliaze delay-per-antenna. Subhanshu et al~\cite{ghaderi2020four} showed that they created a delay element with 0.1 ns resolution with over 6 bit control.
% \cite{boljanovic2021fast} also discusses practical aspects of TTD arrays.

% \cite{park201315,ma2015silicon} recent advances on TTD have greatly reduced the circuit size and improved the accuracy.

% TTD can be generated in electronics~\cite{chu2013true} or  photonics \cite{cao2015advanced,ng1991first} % SatixFy~\cite{sikri2019multi} built a chip for TTD ararys for space and 5G to solve beam squinting issue.


% Now we proceed to describe our algorithm to estimate optimal delays and phases per antenna in real-time.


% However, just using a delay-element would create a linear sweep in frequency-space as shown in Fig.~\ref{fig:delay_per_antenna_fig}b, which allocates only a small number of subcarriers in each direction. It cannot allocate an arbitrary large set of subcarriers to a single user on demand for throughput intensive applications such as VR streaming. Finally, it also puts a constraint on the scheduler with frequency subcarriers tied to specific directions, even if those subcarriers experience poor channel. In other words, delay-elements only limit the flexibility to allocate the best set of subcarriers to a user just because they cannot send those subcarriers to a specified user direction.
% That is we need to be able to tune set of subcarrier frequencies and the direction of the user in the space for each set of subcarriers independently. \todo{Somewhere talk about range and resolution: requirement for our delays. }


% To achieve this independent tunability of frequency and user's direction in space, in \name we for the first time design a \dpa front-end.
% Wherein by using \dpa we can achieve frequency-selectivity from the delay-element as only a subset of frequencies are transmitted to a receiver direction in space, determined by the phase elements.
% So, now this gives us two knobs to control the overall gain pattern of the system to achieve frequency-space independence: the phase and delay elements at each antenna. We saw that the phase knob controls the direction of the beam in space, but cannot create frequency-selectivity on its own. The delay knob on the other hand, creates frequency-selectivity by transmitting various frequency components to different directions, but cannot achieve independence in the 2D domain of frequency-space. 
% For instance, we may want 50\% bands to transmit in one direction and the rest 50\% bands to be transmitted in another direction to serve two users over two frequency bands. 
% That is we need to get a gain pattern profile, which we call a frequency-space image, as shown in Fig.~\ref{fig:delay_per_antenna_fig}(d) wherein frequency and space are independent of each other.
% So we need to estimate the delay and phase values for the \dpa which create independence across the 2D gain pattern profile.
% To understand how we can create these independent frequency-space gain pattern profiles, let us take a look at the gain pattern of this antenna array:

% \begin{equation*}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} U(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% \end{equation*}

% Now to understand how to tune the delay and phase weights, $w_{dpa}(k,n)$, so as to get the desired independent frequency-space profile let us consider a simple example with two users located at $0^\circ$ and $30^\circ$. Suppose we want to send first half frequency subcarriers to the first user and the second half to the second user. 
% Thus we would need to achieve a frequency-space plot as shown in Fig.~\ref{fig:fsda_explain}(d), where the gain pattern must be high at the two desired frequency-space locations corresponding to the two users and must be low at other locations. 

% At a high level, we know that the phase knob shifts the pattern across the space axis and the delay knob controls the slope of frequency-space gain curve. But to be able to create the frequency-space profile shown in Fig.~\ref{fig:fsda_explain}(d), we need to achieve: (R1) `narrower beams' to be able to have minimal inter-user interference, (R2) one set of phase-delay values to provide the required slope to `align' the required frequencies along the required directions, (R3) one set of phase-delay values to provide the required slope to `nullify' the frequencies spread across other directions, (R4) we also need `multiple' of these slopes (equal to the number of users and directions) in a single image to generate an effective image with that number of frequency-space independent beams.


% With these requirements in mind, we solve for the optimal phase-delay values using our algorithm that we describe in the next subsection. But we give a quick intuition on how we achieve the required frequency-space gain profile using our estimated values for the above said example. Firstly, we show two signature images in Fig.~\ref{fig:fsda_explain}(a) and~\ref{fig:fsda_explain}(b). Here we we first demonstrate it using a total of 4 antennas and use the first three antennas to create the first signature image and the last two antennas to create the second signature image. 
% We can observe that using a higher number of antennas create a narrower beam and so the first signature image has a `narrower beam'(R1) than the second image. See how the two images illuminates different regions in the frequency-space grid. The first image illuminate a linear region with a positive slope and the second image consists of `two lines' (R4) with a negative slope such that there is low gain in the middle of those two lines. When these two images are combined together, the power adds up differently in different regions. Some regions `align' to create to higher gain regions (R2) while other regions `nullify' each other leading to low gain regions (R3). The combined response of all 4 antennas is shown in Fig.~\ref{fig:fsda_explain}(c). We see that the constituent images combine together to create this desired response. In fact, if we have more antennas, say 8 of them, then we can get even `sharper' response as shown in Fig.~\ref{fig:fsda_explain}(d) due to higher constructive combining gains. So, in summary, by controlling the phases and knobs of different sub-arrays and the number of antennas in each sub-arrays, we could achieve an arbitrary frequency-space image. 

% This intuition helps in understanding how fundamentally any frequency-space images are created, but it doesn't help yet on what values of delays and phases we should apply at each antenna to create this image or rather how to estimate these values of delays and phases accurately in real-time. So, now we proceed to describe our novel algorithm to estimate optimal delays and phases per antenna in real-time in the next sub-section.

%% New subsection
\subsection{Estimating delays and phases in \dpa}\label{sec:design-est}
To create a desired frequency-direction beam response, the gNB (base station) needs to estimate the corresponding delays and phases per-antenna in \dpa. One naive solution is to try different discrete values in a brute-force way using a look-up table to get the desired beams. But, this solution is computationally hard and memory intensive since there is a large set of possibilities for the delays and phases at each antenna. For instance, with 64 delays and 64 phases per antenna (assume both are 6-bit, so $2^6=64$), a brute-force look-up table search would require $64^N\times 64^N \approx 10^{28}$ probes to try each combination and then storing it all in memory, which is impossible to solve with even high memory and high computing machines. Our insight is that we can pose this problem as an optimization framework and solve them in a computationally efficient way.
% \review{R1: As mentioned by the authors, the bruteforce creation of a look-up table is time-consuming and needs high memory. However, given that this exhaustive process needs to be done only once and the lookup table should be stored at BS (which usually has higher memory and computational power), it's not clear if the proposed optimization algorithm is crucial.} \todo{Ignore this comment. It's obvious that brute-force can't solve the problem.}
% \todo{We call it \algoname algorithm.}

% To understand how we can create these independent frequency-space gain pattern profiles, let us take a look at the gain pattern of this antenna array:

We can now formulate the optimization problem with insights we have obtained from the previous subsection and from the fundamentals of digital signal processing. The goal is to relate weights (delays and phases) to the antenna gain pattern in (\ref{eq:gain}) in a way that simplifies our estimation problem. 
% The gain pattern with \dpa is a function of frequency and space, while the  weights vary over time and antennas. They are related as follows:
% \begin{equation}\label{eq:gain}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) w_\text{dpa}(k,n) V(n,\theta)
% \end{equation}
% % \begin{equation}\label{eq:gain}
% %     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% % \end{equation}
% where $w_{\text{dpa}}(k,n) = \delta(kT_s-\tau_n)e^{j\Phi_n}$ is the antenna weights, $\Ubf(f,k)$ is a traditional discrete domain frequency-time transform (DFT). Now since the signal is actually sampled only discretely with a sampling time of $T_s$, our original delay weight element $w_{\text{delay}}(t,n)$ would reduce to $w_{\text{delay}}(k,n) = \delta(kT_s-\tau_n)$ as described in the above equation.
Our insight is that similar to how frequency and time are related by a Fourier transform, there is a similar transform that relates space and antenna using steering matrices. So, there are two transforms which bridges the two world of antenna weights and desired gain pattern. Mathematically, we represent gain pattern by a discrete frequency-space matrix $\Gbf$ and the weights as discrete time-antenna matrix $\Wbf$ and relate them with the following 2D transform:
\begin{equation}
    \Gbf = \Ubf\Wbf\Vbf
\end{equation}
where $\Ubf$ is time to frequency transform matrix and $\Vbf$ is antenna to space transform matrix. Here we formulate $\Wbf$ as $K\times N$ matrix, where $K$ is the number of discrete time values and $N$ number of antennas. 

We follow a three step process to estimate the weight matrix $\Wbf$ that create our desired frequency-space image intuitively explained in Fig. \ref{fig:algo_fsda_steps}. There are two inputs to our algorithm: Angles and desired frequency bands for each user. These two inputs are enough to represent the given frequency-space image. As a first, we create a binary frequency-space matrix which consists of 1s at desired frequency-space locations and 0s otherwise, we denote it by $\Gbf_{\des}$. We then formulate the following optimization problem:
\begin{equation}
\begin{split}
        \hat{\Phi_n},\hat{\tau_n} &= \min ||\Gbf_\des - \Ubf\Wbf\Vbf||^2\\
        \text{s.t.}\quad &\Wbf(k,n) = e^{j\Phi_n}\delta(kT-\tau_n)
\end{split}
\end{equation}
This optimization is a non-convex due to the non-linear terms such as exponential in phase and delta in delay. Moreover, the constraint on having a discrete set of values for delays and phases makes it NP-hard. We make an approximation by relaxing the delta constraint and letting the weights at each antenna take any variation over time. It means that we allow weights to take the form of a continuous profile over time at each antenna rather than a delta function which is non-zero at only one value and zero otherwise. We call it the delay-phase profile at each antenna. How do we estimate this delay-phase profile?


Our insight is that we can write an inverse transform of $\Ubf$ and $\Vbf$ to go from the frequency-space domain to the time-antenna domain. The logic behind such formulation is that using appropriate discrete grid along time and space axis, we can formulate $\Ubf$ and $\Vbf$ as linear transforms, i.e., $\Ubf^\dagger\Ubf=\Ibf$ and $\Vbf\Vbf^\dagger=\Ibf$ for identity matrix $\Ibf$ (Note $(.)^\dagger$ is pseudo-inverse of a matrix). Therefore, it is easy to write their inverse by simply taking the pseudo-inverse. We estimate $\hat{\Wbf}$ as:
\begin{equation}
    \hat{\Wbf} = \Ubf^{\dagger}\Gbf_\des\Vbf^{\dagger}
\end{equation}
The final step of our algorithm is to extract delays and phases from $\hat{\Wbf}$. Note that each column in $\hat{\Wbf}$ contains the delay-phase profile. We find the maximum peak in this profile, and the index corresponding to this peak gives the delay, and the max value at this peak gives the phase term. Note that since we did not put any restriction on the number of non-zero delay taps, we could get more than one delay tap per antenna. We empirically found that the estimated delay profile has only one significant peak with high magnitude than other local peaks (See Section \ref{sec:evaluation}). Also, the intuition comes from our insights from the previous section that usually, one delay per antenna suffices in creating the desired response. 

\noindent
\textbf{Weights Quantization:} The delay and phase values obtained from our algorithm is still continuous in nature and must be discretized to be fed into the \dpa hardware. We quantize both the phase and delay values with a 6-bit quantizer in software before feeding to the array. The quantized phase takes one of the 64 values in $[0^\circ,360^\circ)$ and quantized delay varies in the range [0, 6.4ns) with an increment of 0.1 ns.


% \subsection{Putting it all together}~\label{sec:design-scheduler}


%  In fact this spectral efficiency can only be realized if the RF-front end design is accompanied by a appropriate scheduler design. While, traditional single beam RF-front end limits the scheduler to schedule users along the same direction. Since, the available range of 

% Traditional single beam scheduler can only schedule users along the same direction. Typically users within same location are made into user groups and at particular instant of time one user group with specific location is served.The challenges here are which user group to schedule and which users to be considered within a group when demand is more than available bandwidth. Here we need to tradeoff between user fairness and overall throughput. In general,
% this approach is inefficient for URLLC scenarios or user groups with low demand. This limitation is mainly due to hard restriction of serving all sub carriers in the same direction.

% In \name, we can schedule multiple users at the same time even if they are located in different directions from the gNB without degrading the SNR performance of the other users. The two challenges for \name are which user groups are to be served in a particular TTI and how many subcarriers to allocate to those users. We create an abstraction with the beam directions, by dividing the space into predefined set of beams in a codebook (beams can be overlapping to avoid corner users) that covers the entire space. We then divide users into groups according to their proximity where each other which can be served via a single designated beam. TDMA approach can only support one user group at a time. In contrast, we propose a scheduler design that can select multiple user groups at a time to serve them according to their demands as shown in Fig. \ref{fig:scheduler_logic_fsda}. 

% The core idea here is enable the flexibility to serve users at different locations in different frequencies, thus truly bringing OFDMA based schedulers into 5G millimter wave ecosystems. \name can accommodate any efficient sub-6 OFDMA schedulers which improves overall throughput, latency and fairness among users. Any existing schedulers in sub-6, such as proportional fair, round-robin, maximum throughput or any other optimal custom schedulers can now be extended to millimeter waves with \name. 


% As a result, by adding new scheduling capabilities, we can support a large number of users with high throughput and low latency, without any limitations or constraints imposed by user location, as opposed to TDMA, which is constrained by user direction, and Split-antenna phased array, which compromises throughput to achieve low-latency FDMA scheduling.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/overview_fsda_scheduler_v2.pdf}
    \caption{Implementation overview for \name with four main components: Data traffic generator, Fast beam scan angle estimation, a scheduler and our \algoname algorithm. The scheduler frequency-multiplex multi-user data in orthogonal set of subcarriers in a single stream per TTI that is sent to the \dpa with a single RF chain. The \algoname algorithm creates appropriate delays and phases to configure the \dpa to radiate only the intended frequency bands to the corresponding user groups.
    }
    \label{fig:overview_fsda_scheduler}
\end{figure}
% End-end design overview of \name with a traffic generator, scheduler, \algoname algorithm and the \dpa mmWave front-end architecture. \textcolor{blue}{We emphasize two phases: 1. Beam scan phase that estimates the angles for all users required for our \algoname algorithm and 2. Data transmission phase, which supports flexible frequency multiplexing by radiating different frequency bands in different directions in a controlled manner. } \review{R1: Finally, the paper uses a single-chain architecture as shown in Fig 3 and Fig 6. The reviewer wonders how independent data streams can be generated and sent to multiple clients if the BS has a single-RF chain architecture. The authors are encouraged to clarify this in the paper.} \todo{Keep on using the term "Frequency multiplexing" and not multi-streaming. Repeat it more often.}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/scheduler_logic_fsda.pdf}
%     \caption{Shows \name's scheduler design with user selection and frequency-space mapping.}
%     \label{fig:scheduler_logic_fsda}
% \end{figure}

==> Arxiv/4_design.tex <==
% !TEX root = main.tex
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fsda_explain.pdf}
    \caption{Explanation on how \dpa creates a desired frequency-space image in (a) with two beams at $0^\circ$ and $30^\circ$. The $0^\circ$ beam occupies frequency range in [-200,0] MHz and $30^\circ$ beam occupies frequency range of [0,200] MHz. Specific frequency-space signatures are shown in (b) and (c) with antenna sub-arrays and final frequency-space image is shown in (d) and (e) with 4 and 8 antennas respectively.}
    \label{fig:fsda_explain}
\end{figure*}

\section{\dpa hardware design} \label{sec:design}
\name designs a new mmWave front-end architecture called \dpa to enable flexible directional frequency multiplexing for mmWave network. 
We have seen in ~\cref{sec:motivation} how the existing mmWave phased array and \ttd array fail to create the desired frequency-direction response. 
% In section~\cref{sec:design-dpa}, we describe how we create such a response with \dpa. We then describe the range and resolution analysis for the delay element in \dpa in ~\cref{sec:design-range} and present our novel algorithm to estimate optimal delays and phases in~\cref{sec:design-est}.  
In this section, we describe \name's architecture and how we program it to create the desired multi-beam response with controllable beam-bandwidth. We then present a range and resolution analysis for the programmable delay element and provide a discussion on the practical implementation of \name and how it generalizes to any arbitrary number of beams, beam-bandwidth, and beam directions.

% \noindent
\subsection{ Architecture of delay-phased array (DPA)} 
\todo{Describe from Figure 2 and focus on simple expression of G(f,theta)}

We now describe intuitively how \dpa creates multi-beam response with arbitrary beam-bandwidth and visualize the frequency-direction patterns that it creates. Let's say we set the phase value $\Phi_n$ and delay value $\tau_n$ at antenna index $n$ (Out of total $N$ antennas in a linear array), the antenna weight weight vector $w_\text{dpa}(n,f)$ is then given by:
\begin{equation}
    w_\text{dpa}(n,f) = e^{j\Phi_n+j2\pi f \tau_n}
\end{equation}
Notice the weight vector is a function of both antenna index $n$ and frequency $f$. Therefore, the beamforming response of this weight vector will also be a function of both frequency and direction.
The beamforming gain of an antenna array is defined as the power radiated by the antenna array in open space. The expression for beamforming gain $G(f,\theta)$ for \name  at a frequency $f$ and direction $\theta$ is given by:
\begin{equation}
\begin{split}
        G(f,\theta)  &= \left\|\sum_{n=0}^{N-1} w_\text{dpa}(n,f) e^{-jn\pi\sin(\theta)}\right\|^2\\
        % &= \sum_{n=0}^{N-1} e^{j\Phi_n+j2\pi f \tau_n} e^{-jn\pi\sin(\theta)}
\end{split}
\end{equation}
Essentially, the response is the sum of the individual contribution from all antennas. Note that we make an approximation above that the distance between antenna elements is the half wavelength (i.e., $d=\frac{\lambda}{2}$), valid for the frequency band of our interest~\cite{benesty2019array}.  

Before we present our approach to achieving these requirements, we would develop intuition about the analog antenna arrays and how phase and delay in the analog antenna create different $G(f,\theta)$ radiation responses. We would then build on intuition to distill it into our architecture. At a high-level, our \dpa consists of delay and phase elements (Fig.~\ref{fig:baseline_architecture_and_heatmap}(d)). Thus, each antenna (index by $n$) weights are contributed by these two elements:
\begin{equation}
    w_{\text{dpa}}(t,n) = w_{\text{phase}}(n)w_{\text{delay}}(t,n)= e^{j\Phi_n}\delta(t-\tau_n)
\end{equation}
The gain pattern with \dpa can be written as a function of frequency and space ($\sin(\theta)$) as:
\begin{equation}\label{eq:gain}
    G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) w_\text{dpa}(k,n) V(n,\theta)
\end{equation}
% \begin{equation}\label{eq:gain}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% \end{equation}
% $w_{\text{dpa}}(k,n) = \delta(kT_s-\tau_n)e^{j\Phi_n}$ is the antenna weights, 
where $\Ubf(f,k)$ is a discrete domain Fourier transform (DFT) and the steering matrix $V(n,\theta)$ is explained before in (\ref{eq:phasedarraygain}). Now since the signal is actually sampled only discretely with a sampling time of $T_s$, our original delay weight element $w_{\text{delay}}(t,n)$ would reduce to $w_{\text{delay}}(k,n) = \delta(kT_s-\tau_n)$ as described in (\ref{eq:gain}).

% \noindent
\subsection{ Range of delay element in \dpa}
It is important to analyze the set of possible delay values that the hardware can support practically. Here we describe the requirements for the delay range and how it helps create a practical circuit board. Delay elements are implemented with variable-length transmission lines on a circuit board. Building large delay lines in IC at mmWave frequencies is prohibitive because of large size, bandwidth, and matching constraints~\cite{ghaderi2019integrated}. Therefore, our design ensures that the delay range is not too large. While traditional true-time delay (TTD) array requires a delay range proportional to the number of antenna $N$, which is large for large antenna array (18.75 ns for 16 antenna array)~\cite{li2022rainbow}. In contrast, the delay range for \name is independent of the number of antennas. For the two-beam case, the delay range for \name is $\frac{3}{2B}$ (derived later in this section), which is $3.7 ns$ for 400 MHz bandwidth for 5G NR; significantly less than that required by TTD arrays. The delay range increases with the number of concurrent beams, but typically 2-3 beams are suitable for practical applications.
% The resolution of \name tells us what step-size of delay value the hardware should support to create desired beams. \name's resolution is obtained as $\frac{\pi\sin(12^o)}{2\pi B} = 0.25 ns$ for minimum beam separation of $12^o$, and 400 MHz system bandwidth. Thus, the requirement for delay range is 3.7 ns and step-size is 0.25 ns. 

Delay control with sub-ns accuracy has been demonstrated in full-duplex circuits for interference cancellation~\cite{nagulu2021full}. Recently, authors of~\cite{ghaderi2020four} have shown accurate delay control with 0.1 ns resolution and with 6-bit control (64 values until 6.4 ns), which satisfies the requirement of \name. 



% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/delay_per_antenna_fig.pdf}
%     \caption{Shows our proposed mmWave system which implements variable delays and phases per-antenna to create frequency-selective beams.}
%     \label{fig:delay_per_antenna_fig}
% \end{figure}

%  \begin{figure} [!t]
%     \subfigure{{\includegraphics[width=0.23\textwidth]{figures/design_delay_range_vs_UEs.pdf}\label{fig:user_variations}}}
%     \subfigure{{\includegraphics[width=0.23\textwidth]{figures/design_delay_range_vs_antennas.pdf}\label{fig:antenna_variations}}}
%     % \subfigure{{\includegraphics[width=0.24\textwidth]{figures/benchmark_convergence.pdf}\label{fig:convergence}}}
%     \caption{Delay range for \name's \dpa with (a) Number of splits/user directions and (b) Number of antennas. Shows average and standard deviation of multiple random trials, each with random set of angles and frequency bands for specific number of user directions. }
%     % \vspace{4pt}
%  \end{figure}

% \review{R2 and R1: It is not clear to me how you can transmit multiple streams to multiple users using a single-chain. Since the delays are only introducing phases, how do we generate different data streams to different users? I am assuming that you have to use multiple chains so as to rtansmit different data streams to different users. If this is the case, would this not be the largest source of complexity in this architecture? why not use M chains each with its own phase array front end and coordinate between the chains in software? Wouldn't that be simpler? I think comparing with these different architectures would be important to understand if the benefits of this work are really validated.} \todo{Explicitly mention "flexible frequency multiplexing" often}.


% Finally, we evaluate \name with a real-time scheduler, traffic generator and \dpa emulation in ~\cref{sec:evaluation} and conclude the paper with a discussion on practical aspects of \dpa.
% We then describe how the new programmable front-end integrates with higher layers in the networking stack in ~\cref{sec:design-real}. 
% We specifically focus on our scheduler design logic which determines which users to serve in each time-slot and over what frequency bands and show the end-to-end system of \name.
% Finally, we conclude by addressing important system-level challenges in building end-to-end system with \name in ~\cref{sec:design-real}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/range_requirement_ttd_vs_dpa.pdf}
%     \caption{\textcolor{blue}{In contrast to true-time delay arrays, our \dpa has lenient delay range requirements which is better feasible to implement in circuits~\cite{ghaderi2019integrated}.}}
%     \label{fig:range_requirement_ttd_vs_dpa}
% \end{figure}

\section{\dpa Software Design for \name}
\subsection{Requirements for \name}


% Before we explain how \dpa works, we first focus on the delay element and show how it enables frequency-selectivity. The delay element creates different delays to the input signal at each antenna before they get radiated in space. When multiple copies of these waveforms from each antenna are added at the receiver, they create a unique gain pattern depending on the frequency content of the signal. To understand it concretely, we define the  antenna weights with delay element as:
% \begin{equation}
%     w_{\text{phase}}(t,n) = \delta(t-\tau_n)
% \end{equation}
% where $\tau_n$ is the variable delay at antenna $n$ and $t$ is the time axis. 

% Here we can intuitively understand that a time varying signal has a certain frequency response. Upon taking FFT of $\delta(t-\tau_n)$, we get $e^{j2\pi f\tau_n}$. We observe that the phase of this exponential term is frequency-dependent, or in other words, the delay element creates frequency-varying phase at each antenna element. Now how does this enables frequency-selectivity? Unlike traditional phased array which adds a constant phase across all frequencies, we see that here different frequency components experience a different phase shift at each antenna which will make them radiate in different directions. 

% A natural question is whether this delay element can create a desired frequency-selective beams. Past work on delay-only array\footnote{Delay-only array is referred as true-time delay array in literature.}~\cite{yan2019wideband, boljanovic2020design,wadaskar20213d,boljanovic2020true,boljanovic2021fast} have shown that this architecture creates a prism-type response by radiating all the frequencies in all the directions in a linear fashion as shown in Fig.~\ref{fig:delay_per_antenna_fig}(b). This response has two major limitations: 1) most frequency bands would be wasted in space if there are no user in that direction and 2) each user gets a small frequency band and cannot scale it up arbitrarily. Due to these limitations, delay-only array is not suitable for our multi-user communication scenario. 

% In \name, for the first time, we show that any arbitrary frequency-space response is achievable with appropriate programming of \dpa. 
% The \dpa architecture consists of a variable delay and a variable phase element at each antenna as shown in Fig.~\ref{fig:baseline_architecture_and_heatmap}(d). So far we have seen that the phase element alone cannot achieve frequency-selectivity and the delay element alone cannot create arbitrary and controlled frequency-selective beams. 
% \subsection{How \dpa creates arbitrary frequency-direction beam response?}\label{sec:design-dpa}

Our goal is to construct arbitrary frequency-direction response $G(f,\theta)$ via an analog antenna array architecture, which would be energy efficient and enable efficient resource utilization and low latency. If we carefully notice the example in section 2, we observe that the split antenna achieves the frequency-direction mapping but with a loss of 6 dB SNR, which is a corollary of the entire 400 MHz radiated in each of the four directions. It leads to our first requirement:   
\noindent
\textbf{Req.1:} \textit{The signal must be transmitted/received in frequency-direction used by users, i.e., each band of frequencies must be radiated only in the direction of users they are associated with, and frequencies not associated with the user-direction must have no energy, i.e., create a null at those frequencies}
Furthermore, we should be able to control the amount of bandwidth assigned to each user, which leads to: 
\noindent
\textbf{Req.2:} \textit{Creating beams narrow in space (for higher antenna gain) but arbitrarily wide in the frequency domain (to support high demand users):}


\subsection{Meeting \name's requirements with \dpa} 


Our insight is to control two knobs: delays $\tau_n$ and phase $\Phi_n$ to get the desired response. 
By taking FFT and equating exponential phase to that of array response, we get: $\Phi_n + 2\pi f \tau_n = n\pi \sin(\theta)$. The variable-delay causes a slope in frequency ($f$) - space ($\sin \theta$) plot, while the variable-phase causes a constant shift along the space axis. Together, they can create an arbitrary line with configurable slope and intercept in frequency-space domain. 

% \noindent
% \textbf{Estimating delay and phase values:}
Now, we ask what set of delays and phases per antenna would give us the beamforming gain pattern with the desired beam-bandwidth and beam direction. We first consider a simple case of two beams with equal beam-bandwidth of $B/2$ each, where $B$ is the total system bandwidth. We assume the two beams are directed along $(-\theta_0, \theta_0)$ respectively as shown in Figure \ref{fig:dpa_proof}(a). We will later discuss a general case with arbitrary beam-bandwidth and beam direction.

We provide a closed-form expression for the set of delays $\tau_n$ and phases $\Phi_n$ for each antenna $n$ ($n=0,1,\ldots,N-1$) that would generate the given beamforming response as follow:
\begin{equation} \label{eq:tau_closed}
    \tau_n = \left(\frac{3}{2B}n\sin(\theta_0)\right)\;\;\;\text{mod }\frac{3}{2B} 
\end{equation}
\begin{equation}\label{eq:phase_closed}
    \Phi_n = 
    \begin{cases}
        0 & \text{when}\;\;\cos(n\pi\sin(\theta_0))> 0 \\
        \pi & \text{when}\;\;\cos(n\pi\sin(\theta_0))<0
    \end{cases}
\end{equation}
We emphasize key takeaways from these expressions before jumping into their proof. Note that the delay values are bounded within a range of $\frac{3}{2B}$ independent of the number of antennas. Within this range, the delay values will monotonically increase or decrease with antenna index $n$, but for large $n$, the delay wraps around with this range factor. 




% We set two \textbf{requirements} for achieving such response: 1) The frequency bands must be transmitted along the user directions and not along other directions where there is no user, i.e., create a null in those directions. 2) Provide a large chunk of frequency bands to each user with narrow beams. We take insights from both both delay-domain and phase-domain to meet these requirements. Basically, delay and phase are two knobs in \dpa and by appropriately tuning these two knobs, we could achieve our desired response. 


% Let's understand it through a simple example with two distinctly located users where we stream half frequency bands to one user and another half to other user. Here the desired frequency-space image will look like shown in Fig.~\ref{fig:delay_per_antenna_fig}(d). How should we set the delays and phases to achieve this response? For simplicity, lets first consider only two antennas with relative delay $\Delta\tau$ and relative phase $\Delta\Phi$. Our main insight is that the delay causes a slope in frequency-space domain, while the phase causes a constant shift in space domain. Together, they can create an arbitrary line with configurable slope and intercept in frequency-space domain.

With this intuition in place, we revisit and explain how can \name achieve these requirements through a simple two-user example in Fig.~\ref{fig:fsda_explain}. Let us consider the two users are located at $0^\circ$ and $30^\circ$ respectively, and the base station wishes to serve these two users over two different frequency bands in a single timeslot. To support such flexible directional frequency multiplexing, the base station must create a frequency-direction beam response shown in Fig.~\ref{fig:fsda_explain}(a). We call such 2D beam patterns as \textit{frequency-space images} for simplicity. So how does \dpa create these images and meet the above requirements? 

% Let us take a simple example how we create a desired frequency-space image in Fig.~\ref{fig:fsda_explain}(d) with two distinctly located users where we stream half frequency bands to one user and another half to other user. We define two requirements for creating such response as follows:
We achieve these requirements by assigning two antenna sub-arrays of the given antenna array to create complementary responses as shown in Fig.~\ref{fig:fsda_explain}(b) and (c), respectively. The first sub-array uses the first three antennas to create a frequency-space image with a positive slope, while the second sub-array creates a negative slope. We can achieve a positive or negative slope by increasing or decreasing delay values at consecutive antennas. Also, note there are two slopes in Fig.~\ref{fig:fsda_explain}(c) due to aliasing. It happens when relative delay between antenna is larger than $\frac{1}{B}$~\cite{li2022rainbow} and is akin to aliasing due to $d>\frac{\lambda}{2}$ in standard phased arrays~\cite{benesty2019array}. 
% \footnote{Fig.~\ref{fig:fsda_explain}(b) shown two slopes in frequency-space image which can be explained by aliasing feature in phased array. Interested readers are directed to~\cite{benesty2019array} for more details on aliasing}. 
When the two responses are combined together, we observe a frequency-space image in Fig.~\ref{fig:fsda_explain}(d) that they combine constructively at desired user locations while creating a null (low gain) at other locations (Meeting \textbf{Req-1}). 

For the second requirement, we create such beams by choosing the number of antennas in each sub-arrays. More antenna in a sub-array makes the corresponding signature image narrow in space. For instance, it is easy to visualize from Fig.~\ref{fig:fsda_explain}(b) and (c) that the former response is narrow in space (obtained with 3 antennas) and the later is wider in space (obtained with 2 antennas). In fact, if we have more antennas, say 8 of them, then we can get an even `sharper' response as shown in Fig.~\ref{fig:fsda_explain}(e) due to higher constructive combining gains. So, in summary, we could achieve an arbitrary frequency-space image by controlling the variable phases and variable-delay knobs of different sub-arrays and the number of antennas in each sub-arrays. 

This intuition helps in understanding how fundamentally any frequency-space image can be created, but it does not help yet on what values of delays and phases we should apply at each antenna to create this image or rather how to estimate these values of delays and phases accurately in real-time. We develop a novel algorithm to estimate delays and phases in real-time in section \ref{sec:design-est}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/algo_fsda_steps.pdf}
    \caption{Three steps of our \algoname algorithm to estimate per-antenna delays and phases that generate a desired frequency-space image. The core step is our novel 2D FSDA transform with some pre-processing and post-processing of inputs and outputs respectively. }
    \label{fig:algo_fsda_steps}
\end{figure*}




% \subsection{Variable-Delay's Range and Resolution}\label{sec:design-range}
% Before moving to real-time tuning, one final piece of puzzle with \dpa architecture is to determine what ranges of delays the hardware must support to create the desired frequency-direction response. The variable delay's range depends on the system bandwidth and the array field-of-view, i.e., the maximum angular range of the array. The choice of variable-delay per-antenna for a given bandwidth and angular FoV can be obtained by equating the antenna phase to the phase of the steering vector as: $2\pi f \tau = \pi\sin(\theta)$. This gives, the range of $\tau = \frac{\pi}{2\pi 400e6}=1.25 ns$ per-element for 400 MHz bandwidth and angular range of 90$^\circ$, i.e. the maximum relative delay between any two antenna element is $1.25$ ns. 


% The total range of delays depends on the total number of antennas and the number of concurrent beams created by the \dpa. To understand this relationship, we performed empirical evaluation with varying number of user directions and antennas in Fig.~\ref{fig:user_variations}, and \ref{fig:antenna_variations} respectively. We observe that \name's \dpa has a lenient requirement on the range of delay values. For instance, the range of delay for \ttd array is $1.25(N-1) ns = 18.75 ns$ for $N = 16$ elements in a uniform linear array~\cite{yan2019wideband, boljanovic2020design,boljanovic2020true,boljanovic2021fast} which increases linearly with number of antennas. Such large delay values is hard to create in circuits due to high losses in transmission lines~\cite{ghaderi2019integrated}.  

% In contrast, the delay range in \dpa is independent of the number of antennas for large antenna arrays. For instance, with 16 antennae or higher and 4 simultaneous beams, \dpa requires a range of $8.75$ns, which is smaller than true-time delay arrays. The reason why we require less delay range comes from our Requirement-1 of creating nulls in frequency-space images. The null is created using a large negative relative delay (to create beams with negative slope and aliasing in the second sub-array as shown in Fig.~\ref{fig:fsda_explain}(c)), which resets the continuously increasing delay of the first sub-array. Thus, the \dpa range is lower than that of true-time delay arrays, which do not create any nulls.


% Similarly, we can obtain the resolution in the variable delay values that represents the minimum step-size in delay variation the hardware should support. The delay resolution is obtained as $\frac{0.2\pi}{2\pi 400e6} = 0.25$ns for the beam width of $\sin(12^\circ)=0.2$. 

% In summary, the \dpa must provide a range of 8.75 ns with the step-size of 0.25 ns for the variable-delay element. These delays can be implemented in the IF stage of the phased array, with the required resolution and minimal power loss. Delays with sub-ns control have been demonstrated for full-duplex wireless applications~\cite{nagulu2021full,mondal20172,garakoui2015compact} which use the delay effect to mimic the self-interference channel. Recently,~\cite{boljanovic2021fast,park201315,ma2015silicon,ghaderi2020four} have combined accurate delay elements with arrays in commercial grade RFICs. Additionally, in~\cite{ghaderi2020four}, the authors develop a 0.1 ns resolution delay element with 6 bits of range control, well within the requirements of our system. In \name, we propose to repurpose these delays to create the desired frequency-direction response for flexible directional frequency multiplexed mmWave communications.


% delay in IF and 1. How practical phased arrays reliaze delay-per-antenna. Subhanshu et al~\cite{ghaderi2020four} showed that they created a delay element with 0.1 ns resolution with over 6 bit control.
% \cite{boljanovic2021fast} also discusses practical aspects of TTD arrays.

% \cite{park201315,ma2015silicon} recent advances on TTD have greatly reduced the circuit size and improved the accuracy.

% TTD can be generated in electronics~\cite{chu2013true} or  photonics \cite{cao2015advanced,ng1991first} % SatixFy~\cite{sikri2019multi} built a chip for TTD ararys for space and 5G to solve beam squinting issue.


% Now we proceed to describe our algorithm to estimate optimal delays and phases per antenna in real-time.


% However, just using a delay-element would create a linear sweep in frequency-space as shown in Fig.~\ref{fig:delay_per_antenna_fig}b, which allocates only a small number of subcarriers in each direction. It cannot allocate an arbitrary large set of subcarriers to a single user on demand for throughput intensive applications such as VR streaming. Finally, it also puts a constraint on the scheduler with frequency subcarriers tied to specific directions, even if those subcarriers experience poor channel. In other words, delay-elements only limit the flexibility to allocate the best set of subcarriers to a user just because they cannot send those subcarriers to a specified user direction.
% That is we need to be able to tune set of subcarrier frequencies and the direction of the user in the space for each set of subcarriers independently. \todo{Somewhere talk about range and resolution: requirement for our delays. }


% To achieve this independent tunability of frequency and user's direction in space, in \name we for the first time design a \dpa front-end.
% Wherein by using \dpa we can achieve frequency-selectivity from the delay-element as only a subset of frequencies are transmitted to a receiver direction in space, determined by the phase elements.
% So, now this gives us two knobs to control the overall gain pattern of the system to achieve frequency-space independence: the phase and delay elements at each antenna. We saw that the phase knob controls the direction of the beam in space, but cannot create frequency-selectivity on its own. The delay knob on the other hand, creates frequency-selectivity by transmitting various frequency components to different directions, but cannot achieve independence in the 2D domain of frequency-space. 
% For instance, we may want 50\% bands to transmit in one direction and the rest 50\% bands to be transmitted in another direction to serve two users over two frequency bands. 
% That is we need to get a gain pattern profile, which we call a frequency-space image, as shown in Fig.~\ref{fig:delay_per_antenna_fig}(d) wherein frequency and space are independent of each other.
% So we need to estimate the delay and phase values for the \dpa which create independence across the 2D gain pattern profile.
% To understand how we can create these independent frequency-space gain pattern profiles, let us take a look at the gain pattern of this antenna array:

% \begin{equation*}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} U(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% \end{equation*}

% Now to understand how to tune the delay and phase weights, $w_{dpa}(k,n)$, so as to get the desired independent frequency-space profile let us consider a simple example with two users located at $0^\circ$ and $30^\circ$. Suppose we want to send first half frequency subcarriers to the first user and the second half to the second user. 
% Thus we would need to achieve a frequency-space plot as shown in Fig.~\ref{fig:fsda_explain}(d), where the gain pattern must be high at the two desired frequency-space locations corresponding to the two users and must be low at other locations. 

% At a high level, we know that the phase knob shifts the pattern across the space axis and the delay knob controls the slope of frequency-space gain curve. But to be able to create the frequency-space profile shown in Fig.~\ref{fig:fsda_explain}(d), we need to achieve: (R1) `narrower beams' to be able to have minimal inter-user interference, (R2) one set of phase-delay values to provide the required slope to `align' the required frequencies along the required directions, (R3) one set of phase-delay values to provide the required slope to `nullify' the frequencies spread across other directions, (R4) we also need `multiple' of these slopes (equal to the number of users and directions) in a single image to generate an effective image with that number of frequency-space independent beams.


% With these requirements in mind, we solve for the optimal phase-delay values using our algorithm that we describe in the next subsection. But we give a quick intuition on how we achieve the required frequency-space gain profile using our estimated values for the above said example. Firstly, we show two signature images in Fig.~\ref{fig:fsda_explain}(a) and~\ref{fig:fsda_explain}(b). Here we we first demonstrate it using a total of 4 antennas and use the first three antennas to create the first signature image and the last two antennas to create the second signature image. 
% We can observe that using a higher number of antennas create a narrower beam and so the first signature image has a `narrower beam'(R1) than the second image. See how the two images illuminates different regions in the frequency-space grid. The first image illuminate a linear region with a positive slope and the second image consists of `two lines' (R4) with a negative slope such that there is low gain in the middle of those two lines. When these two images are combined together, the power adds up differently in different regions. Some regions `align' to create to higher gain regions (R2) while other regions `nullify' each other leading to low gain regions (R3). The combined response of all 4 antennas is shown in Fig.~\ref{fig:fsda_explain}(c). We see that the constituent images combine together to create this desired response. In fact, if we have more antennas, say 8 of them, then we can get even `sharper' response as shown in Fig.~\ref{fig:fsda_explain}(d) due to higher constructive combining gains. So, in summary, by controlling the phases and knobs of different sub-arrays and the number of antennas in each sub-arrays, we could achieve an arbitrary frequency-space image. 

% This intuition helps in understanding how fundamentally any frequency-space images are created, but it doesn't help yet on what values of delays and phases we should apply at each antenna to create this image or rather how to estimate these values of delays and phases accurately in real-time. So, now we proceed to describe our novel algorithm to estimate optimal delays and phases per antenna in real-time in the next sub-section.

%% New subsection
\subsection{\algoname algorithm for estimating delays and phases in \dpa}\label{sec:design-est}
To create  a desired frequency-direction beam response, the gNB (basestation) needs to estimate the corresponding delays and phases per-antenna in \dpa. One naive solution is to try different discrete values in a brute-force way using a look-up table to get the desired beams. But, this solution is computationally hard and memory intensive since there is a large set of possibilities for the delays and phases at each antenna. For instance, with 64 delays and 64 phases per-antenna (assume both are 6-bit, so $2^6=64$), a brute-force look-up table search would require $64^N\times 64^N \approx 10^{28}$ probes to try each combination and then storing it all in memory, which is impossible to solve with even high memory and high computing machines. Our insight is that we can pose this problem as an optimization framework and solve them in computationally efficient way.
% \review{R1: As mentioned by the authors, the bruteforce creation of a look-up table is time-consuming and needs high memory. However, given that this exhaustive process needs to be done only once and the lookup table should be stored at BS (which usually has higher memory and computational power), it's not clear if the proposed optimization algorithm is crucial.} \todo{Ignore this comment. It's obvious that brute-force can't solve the problem.}
% \todo{We call it \algoname algorithm.}

% To understand how we can create these independent frequency-space gain pattern profiles, let us take a look at the gain pattern of this antenna array:

We can now formulate the optimization problem with insights we have obtained from the previous subsection and from the fundamentals of digital signal processing. The goal is to relate weights (delays and phases) to the antenna gain pattern in (\ref{eq:gain}) in a way that simplifies our estimation problem. 
% The gain pattern with \dpa is a function of frequency and space, while the  weights vary over time and antennas. They are related as follows:
% \begin{equation}\label{eq:gain}
%     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) w_\text{dpa}(k,n) V(n,\theta)
% \end{equation}
% % \begin{equation}\label{eq:gain}
% %     G(f,\theta) = \sum_{k = 0}^{K-1} \sum_{n=0}^{N-1} \Ubf(f,k) \underbrace{w_{\text{delay}}(k,n)w_{\text{phase}}(n)}_{w_{dpa}(k,n)} V(n,\theta)
% % \end{equation}
% where $w_{\text{dpa}}(k,n) = \delta(kT_s-\tau_n)e^{j\Phi_n}$ is the antenna weights, $\Ubf(f,k)$ is a traditional discrete domain frequency-time transform (DFT). Now since the signal is actually sampled only discretely with a sampling time of $T_s$, our original delay weight element $w_{\text{delay}}(t,n)$ would reduce to $w_{\text{delay}}(k,n) = \delta(kT_s-\tau_n)$ as described in the above equation.
Our insight is that similar to how frequency and time are related by a Fourier transform, there is a similar transform that relates space and antenna using steering matrices. So, there are two transforms which bridges the two world of antenna weights and desired gain pattern. Mathematically, we represent gain pattern by a discrete frequency-space matrix $\Gbf$ and the weights as discrete time-antenna matrix $\Wbf$ and relate them with the following 2D transform:
\begin{equation}
    \Gbf = \Ubf\Wbf\Vbf
\end{equation}
where $\Ubf$ is time to frequency transform matrix and $\Vbf$ is antenna to space transform matrix. Here we formulate $\Wbf$ as $K\times N$ matrix, where $K$ is the number of discrete time values and $N$ number of antennas. 

We follow a three step process to estimate the weight matrix $\Wbf$ that create our desired frequency-space image intuitively explained in Fig. \ref{fig:algo_fsda_steps}. There are two inputs to our algorithm: Angles and desired frequency bands for each user. These two inputs are enough to represent the given frequency-space image. As a first, we create a binary frequency-space matrix which consists of 1s at desired frequency-space locations and 0s otherwise, we denote it by $\Gbf_{\des}$. We then formulate the following optimization problem:
\begin{equation}
\begin{split}
        \hat{\Phi_n},\hat{\tau_n} &= \min ||\Gbf_\des - \Ubf\Wbf\Vbf||^2\\
        \text{s.t.}\quad &\Wbf(k,n) = e^{j\Phi_n}\delta(kT-\tau_n)
\end{split}
\end{equation}
This optimization is a non-convex due to the non-linear terms such as exponential in phase and delta in delay. Moreover, the constraint on having a discrete set of values for delays and phases makes it NP hard. We make an approximation by relaxing the delta constraint and let the weights at each antenna take any variation over time. It means that we allow weights to take the form of a continuous profile over time  at each antenna rather than a delta function which is non-zero at only one value and zero otherwise. We call it delay-phase profile at each antenna. How do we estimate this delay-phase profile?


Our insight is that we can write an inverse transform of $\Ubf$ and $\Vbf$ to go from frequency-space domain to time-antenna domain. The logic behind such formulation is that using appropriate discrete grid along time and space axis, we can formulate $\Ubf$ and $\Vbf$ as linear transforms, i.e., $\Ubf^\dagger\Ubf=\Ibf$ and $\Vbf\Vbf^\dagger=\Ibf$ for identity matrix $\Ibf$ (Note $(.)^\dagger$ is pseudo-inverse of a matrix). Therefore, it is easy to write their inverse by simply taking the psuedo-inverse. We estimate $\hat{\Wbf}$ as:
\begin{equation}
    \hat{\Wbf} = \Ubf^{\dagger}\Gbf_\des\Vbf^{\dagger}
\end{equation}
The final step of our algorithm is to extract delays and phases from $\hat{\Wbf}$. Note that each column in $\hat{\Wbf}$ contains the delay-phase profile. We find the maximum peak in this profile and the index corresponding to this peak gives the delay and the max value at this peak gives the phase term. Note that since we did not put any restriction on the number of non-zero delay taps, we could get more than one delay-taps per-antenna. We empirically found that the estimated delay profile has only one significant peak with high magnitude than other local peaks (See Section \ref{sec:evaluation}). Also, the intuition comes from our insights from previous section that usually one delay per-antenna suffice in creating the desired response. 

\noindent
\textbf{Weights Quantization:} The delay and phase values obtained from our algorithm is still continuous in nature and must be discretized to be fed into the \dpa hardware. We quantize both the phase and delay values with a 6-bit quantizer in software before feeding to the array. The quantized phase takes one of the 64 values in $[0^\circ,360^\circ)$ and quantized delay varies in the range [0, 6.4ns) with an increment of 0.1 ns.


% \subsection{Putting it all together}~\label{sec:design-scheduler}


%  In fact this spectral efficiency can only be realized if the RF-front end design is accompanied by a appropriate scheduler design. While, traditional single beam RF-front end limits the scheduler to schedule users along the same direction. Since, the available range of 

% Traditional single beam scheduler can only schedule users along the same direction. Typically users within same location are made into user groups and at particular instant of time one user group with specific location is served.The challenges here are which user group to schedule and which users to be considered within a group when demand is more than available bandwidth. Here we need to tradeoff between user fairness and overall throughput. In general,
% this approach is inefficient for URLLC scenarios or user groups with low demand. This limitation is mainly due to hard restriction of serving all sub carriers in the same direction.

% In \name, we can schedule multiple users at the same time even if they are located in different directions from the gNB without degrading the SNR performance of the other users. The two challenges for \name are which user groups are to be served in a particular TTI and how many subcarriers to allocate to those users. We create an abstraction with the beam directions, by dividing the space into predefined set of beams in a codebook (beams can be overlapping to avoid corner users) that covers the entire space. We then divide users into groups according to their proximity where each other which can be served via a single designated beam. TDMA approach can only support one user group at a time. In contrast, we propose a scheduler design that can select multiple user groups at a time to serve them according to their demands as shown in Fig. \ref{fig:scheduler_logic_fsda}. 

% The core idea here is enable the flexibility to serve users at different locations in different frequencies, thus truly bringing OFDMA based schedulers into 5G millimter wave ecosystems. \name can accommodate any efficient sub-6 OFDMA schedulers which improves overall throughput, latency and fairness among users. Any existing schedulers in sub-6, such as proportional fair, round-robin, maximum throughput or any other optimal custom schedulers can now be extended to millimeter waves with \name. 


% As a result, by adding new scheduling capabilities, we can support a large number of users with high throughput and low latency, without any limitations or constraints imposed by user location, as opposed to TDMA, which is constrained by user direction, and Split-antenna phased array, which compromises throughput to achieve low-latency FDMA scheduling.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/overview_fsda_scheduler_v2.pdf}
    \caption{Implementation overview for \name with four main components: Data traffic generator, Fast beam scan angle estimation, a scheduler and our \algoname algorithm. The scheduler frequency-multiplex multi-user data in orthogonal set of subcarriers in a single stream per TTI that is sent to the \dpa with a single RF chain. The \algoname algorithm creates appropriate delays and phases to configure the \dpa to radiate only the intended frequency bands to the corresponding user groups.
    }
    \label{fig:overview_fsda_scheduler}
\end{figure}
% End-end design overview of \name with a traffic generator, scheduler, \algoname algorithm and the \dpa mmWave front-end architecture. \textcolor{blue}{We emphasize two phases: 1. Beam scan phase that estimates the angles for all users required for our \algoname algorithm and 2. Data transmission phase, which supports flexible frequency multiplexing by radiating different frequency bands in different directions in a controlled manner. } \review{R1: Finally, the paper uses a single-chain architecture as shown in Fig 3 and Fig 6. The reviewer wonders how independent data streams can be generated and sent to multiple clients if the BS has a single-RF chain architecture. The authors are encouraged to clarify this in the paper.} \todo{Keep on using the term "Frequency multiplexing" and not multi-streaming. Repeat it more often.}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/scheduler_logic_fsda.pdf}
%     \caption{Shows \name's scheduler design with user selection and frequency-space mapping.}
%     \label{fig:scheduler_logic_fsda}
% \end{figure}

==> Arxiv/4_puttingtogether.tex <==
% !TEX root = main.tex
% \subsection{Scheduler Design} \label{sec:design2}

\section{Putting it all together}~\label{sec:design-real}




We have seen how \name's \dpa front-end design enables multi-beamforming across frequency and space, we now describe the overall working of \name in this section, a flowchart of the same is shown in Figure \ref{fig:overview_fsda_scheduler}. 
At a high level, our system needs to firstly perform a fast beam scan to estimate user angles, and provide this information to both our scheduler and \algoname. The scheduler decides which users to serve in the current TTI and over what frequency bands. The \algoname algorithm then estimate delay and phase values to generate appropriate frequency-space beams to serve all the users in that TTI. 

% Our scheduler and \algoname algorithm runs in software to then estimate the user scheduling and appropriate phase and delay control estimates that meet these user scheduling requirements. Finally, these delay and phase controls and the data for that TTI are streamed over to the \dpa front end that can serve selective-frequency resources to multiple users along multiple directions simultaneously.
\noindent\textbf{Fast beam training to get angles:} We leverage existing 5G NR SSB beam scan~\cite{3gpp2020} using exhaustive search to estimate angles. The gNB scans 64 beams in the codebook and each UE reports the best beam index that maximises the received signal strength. The gNB can infer the user's angle from the beam index. Note that \name is agnostic to any beam training scheme as long as it can provide an estimate of user's angle.

% for fast-beam scanning within which it measures the received signal strength in each direction and predicts accurate user direction. Thus, we can use this fast beam-scanning enabled in 5G NR protocol without making any changes and get individual user's directions for \name's end-to-end system deployment.

\noindent\textbf{Scheduler:}
The discrete sectorization of the beam scans result in multiple users to fall into the same spatial sector as seen in Figure~\ref{fig:scheduler_logic_fsda}, these users are usually grouped. Thus now the traditional beam scheduler has a limited flexibility of being able to schedule users along the same direction in a single TTI. In general, this approach is inefficient for URLLC scenarios or scenarios when there are user groups with low demand. This limitation is mainly due to hard restriction of serving all sub-carriers in the same direction.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/scheduler_logic_fsda.pdf}
    \caption{Shows \name's scheduler design with user selection and frequency-space mapping.}
    \label{fig:scheduler_logic_fsda}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/experiment_setup.pdf}
    \caption{We evaluate \name in two indoor conference room settings and outdoors. Figure shows one of our indoor scenario and various components of our phased arrays and the baseband platform. We use our hardware setup to collect channel data at 100s of user locations.}
    \label{fig:experiment_setup}
\end{figure*}

In contrast the \dpa design of \name enables scheduler more flexibility to schedule multiple users/user-groups located along multiple-directions or multiple groups of directions without degrading the SNR performance. 
The core advantage for \name's design is that we can enable the flexibility to serve users at different locations in different frequencies, thus truly bringing OFDMA based schedulers into 5G millimter wave ecosystems. \name can accommodate any efficient sub-6 OFDMA schedulers which improves overall throughput, latency and fairness among users. Any existing schedulers in sub-6, such as proportional fair, round-robin, maximum throughput or any other optimal custom schedulers can now be extended to millimeter waves with \name. 

So, the two biggest challenges that \dpa front end design poses two challenges for \name's scheduler design which are (a) which users or user groups are to be served in a particular TTI and (b) how many subcarriers to allocate to those users. To solve for these firstly, we create an abstraction with the beam directions, by dividing the space into predefined set of beams in a codebook (beams can be overlapping to avoid corner users) that covers the entire space. We then divide users into groups according to their proximity where each other which can be served via a single designated beam. So, we propose a scheduler design that can select multiple user groups at a time to serve them according to their demands as shown in Figure \ref{fig:scheduler_logic_fsda}. 

% \noindent\textbf{Fast beam training to get angles:} We need to know the user's directions at both the schduler and the \algoname to schedule appropriately. To that extent we note that the existing 5G NR protocol~\cite{3gpp2020} already enables for fast-beam scanning within which it measures the received signal strength in each direction and predicts accurate user direction. Thus, we can use this fast beam-scanning enabled in 5G NR protocol without making any changes and get individual user's directions for \name's end-to-end system deployment.
% \textbf{End-end design overview}\\
% Describe overview in Figure \ref{fig:overview_fsda_scheduler}.

% \noindent
% \textbf{Fast beam training to get angles}\\
% \todo{Describe beam training process.}

% \textbf{User mobility management and blockage mitigation is scalable to multiple simultaneous users with \dpa}

% Millimeter-wave directional links are prone to user mobility and blockages which causes degradation in link quality. Most of the current literature is focused on user tracking and blockage mitigation approaches with a single user scenario. Many of these approaches doesn't work with multi-user scenarios, as the they pose a new set of challenges and scale the existing problems severity. \name alleviates this challenges by serving multiple user groups in different directions and enabling additional scheduling features.

% % While serving the user groups, TDMA loses its throughput gains even if one of high demand user link is degraded because of blockage or mobility. \name handles blocakage and mobility in an efficient way compared to the other baselines as only subcarriers in one direction are affected while other directions remain stable. For instance, consider a scenario with 3 users where there demand are 100, 500, 424 subcarriers respectively. here first two users are in one location and third user is different location. TDMA can either support first two users or third user since they are different directions. since first two users demand is more 600(100 + 500), it will serve user group with first two users. if user 2 link is degraded with mobility or blockage, TDMA can only serve 100 subcarriers effectively, lost the 500 subcarriers users. Where as \name simultaneously support both directions serving 1024 subcarriers. even if user-2 link is degraded, it can still support 524 subcarriers reliably. While also use additional beam to track User-2 and regain the link.

%  In general at a high level, the most acceptable solution for blockage and mobility is to search for alternate beam direction towards new user location (via direct or reflected paths) and serve the user through the new beams. Ideally, when one user undergoes blockage or mobility, we do not want other users to suffer in terms of their link throughput. But, traditional split antenna system prohibits smart beam tracking algorithm due to its irregular beam pattern. Since we create independent directional beams towards each user, we can easily track this beam under user mobility. With blockages, we can search a new beam towards a user and switch the beam without disturbing the flow of other users. This is possible because the frequency subcarriers allocated to the user are independent of the user direction, i.e., those subcarriers can be rerouted towards a new user direction easily without affecting the link for other users. This allows smart blockage and mobility management algorithms to scale to a large number of simultaneous users. 

==> Arxiv/5_implementation.tex <==
% !TEX root = main.tex
\section{Implementation}\label{sec:implementation}



We evaluate \name with a combination of simulation and emulation with our 28 GHz phased arrays hardware setup. Our phased arrays consists of 32 elements (8 horizontal $\times$ 4 vertical) each connected to a phase shifter (6 bit resolution or $2^6 = 64$ phase values in $2\pi$). Since delay-phased arrays are not yet commercially available, we devise a emulation based study using commercial phased arrays to evaluate the performance of our algorithm. This is an acceptable practice in research community how phased arrays were emulated using mechanical horn antennas during the early phase of mmWave research~\cite{sur2016beamspy, sur201560, wei2015mtrack, sun2013multi, rappaport201238}. Albeit, a single delay element IC is recently created in academic research~\cite{ghaderi2020four,boljanovic2021fast,mondal20172} and its usability and wide range of applications shows a promising trend for its adoption in near future~\cite{yan2019wideband, boljanovic2020design,wadaskar20213d,tan2019delay}. 

We collect per-antenna channel from each antenna element using a method similar to ACO~\cite{palacios2018adaptive} for performance evaluation in realistic mmWave environment. Note that our algorithm does not require the per-antenna channel estimates for the delay and phase estimation. We only require the angle of user direction which we obtain through an exhaustive beam sweep procedure. We estimate the delays and phases for a given gNB/user location, emulate these delays in software and evaluate the performance of our algorithm and baselines on the measured channel dataset. Our measurement setup is described as follows.\\
\noindent
\textbf{gNB Setup:} We setup a  phased arrays at gNB as shown in (Figure~\ref{fig:experiment_setup}). Each phased array covers a FoV of $120^\circ$ Field-of-view with $12^\circ$ wide half-power beamwidth).  We used USRP X410 since it can support 5G NR specs.

\noindent
\textbf{UE setup:} On the UE side, we use a single phased array connected to X410. We sequentially placed the UE at 50 different locations to collect the channel measurements at different physical location in space and we repeat the process in two different indoor environments. Note that this way of per-user channel data collection allows us to emulate a large combination of simultaneous users by randomly selecting a subset of users in our dataset (e.g., we have $50 \choose 4$ $\approx$ 200k scenarios with 4 simultaneous users).

\noindent
\textbf{Communication model:} Since wireless channel is reciprocal (uplink and downlink take the same physical paths from the transmitter to the receiver). Our goal is to measure the  mmWave channel and we choose uplink channel measurement for its simplicity. We set the UE to always transmit 5G NR reference signals in repeat mode through a quasi-Omni beam, while the gNB receives the signal through various combinations of antennas and beam directions. We create 5G NR compliant waveforms with 120kHz subcarrier spacing over a bandwidth of up to 400 MHz.
% \footnote{USRP X410 can provide up to 400MHz sampling rate, but such high rates were not officially supported at the time of writing.}.


% \subsection{Ground Truth channel collection with ACO-like algorithm and Emulation based study}
% \todo{Describe how we emulate \dpa with real-world mmWave channel measurements with our phased arrays}

% \subsection{Emulation based study}

% \subsection{Hardware description}
% We use two phased array and generate delays in software with 8-tap filter since we have 8 antennas in one phased array. Show that our 8-tap filter is equivalent to 8 delays per-antenna. We have to do this because of limitation of our phased arrays. There are no delay-phased ararys in market. But \cite{ghaderi2020four} have shown a delay element for TTD phased array and this is the future of mmWave phased arrays.

% \todo{Describe our phased arrays}
% % Hybrid architecture inspired by \cite{miao2016joint} where 3 phased ararys are pointing radially different direction each covering 360 space.
% \noindent
% \textbf{Baselines}
% We use the following baselines \todo{Update a description on baselines}


